A Verified Compiler for Quantum Simulation

Hamiltonian simulation is a central application of quantum computing, with significant potential in modeling physical systems and solving complex optimization problems. Existing compilers for such simulations typically focus on low-level representations based on Pauli operators, limiting programmability and offering no formal guarantees of correctness across the compilation pipeline. We introduce QBlue, a high-level, formally verified framework for compiling Hamiltonian simulations. QBlue is based on the formalism of second quantization, which provides a natural and expressive way to describe quantum particle systems using creation and annihilation operators. To ensure safety and correctness, QBlue includes a type system that tracks particle types and enforces Hermitian structure. The framework supports compilation to both digital and analog quantum circuits and captures multiple layers of semantics, from static constraints to dynamic evolution. All components of QBlue, including its language design, type system, and compilation correctness, are fully mechanized in the Rocq proof framework, making it the first end-to-end verified compiler for second-quantized Hamiltonian simulation.

==> background.tex <==
\section{Overview}
\label{sec:background}

This section provides an overview of \qsnd, with some background information. In-depth background information is in \Cref{app:paulimap}.

%\vspace*{-0.3em}
\subsection{Quantum State Representation}\label{sec:background1}
%\vspace*{-0.3em}

In this section, we introduce the state representation for \emph{quantum particle systems}, where a quantum computer admits a special kind of particle system, a.k.a., \emph{quantum qubit states}, with each site being a two-dimensional Hilbert space $\Hilb_2$.

We first examine the necessary components in particle system states.
A quantum particle system has finite $n$ sites, and each site might have different dimensionalities, i.e., bosons and fermions might require different Hilbert space dimensionalities to represent them. For example, in a three particle system, we might want to assume that the first particle state is modeled as $\Hilb_3$, the second one is $\Hilb_4$, and the last one is $\Hilb_5$ ($3 * 4 * 5$); therefore, the whole system is a 60 dimensional Hilbert space $\Hilb_{60}$.
%
The above can be viewed as the composition of the three particle states as $\Hilb_{3}\otimes \Hilb_{4}\otimes \Hilb_{5}$; each position in the tensor refers to the Hilbert space region storing the quantum information for the different particles. 

To represent the state, we propose \emph{typed Hilbert space states} for our quantum state representation \footnote{Theoretically, a typical particle system simulation is defined in terms of fock state, an infinite direct sum of Hilbert spaces $\bigoplus_{n=0}^{\infty} \Hilb^n$. Practical quantum particle computation approximates the Fock state representation using a finite Hilbert space.}
The whole quantum state of an $n$ particle system is a composition of different site states, as $\Hilb_{N}=\bigotimes_{j=0}^n \Hilb_{m_j}$. Each site state is an $m_j$ dimensional Hilbert space $\Hilb_{m_j}$, classicied as a type $t(m_j)$ (or $t^{\aleph}(m_j)$ for fermions) state.
A $\Hilb_{m}$ space vector is $\begin{psmallmatrix} z_0 \\ z_1 \\ ... \\ z_{m\sminus 1} \end{psmallmatrix}$, where the \emph{amplitudes} ($z_j$) are complex numbers; in a \emph{normalized particle state}, $\sum_{j=0}^m |z_j|^2 = 1$.
The dimension of the whole quantum state is defined as $N=\Pi_{j=0}^n m_j$.
Specifically, if every particle is $t(2)$ typed, the system becomes a \emph{qubit system}.
Note that our state representation assumes that an $m$-dimensional Hilbert space can be constructed for a single particle, which is typically constructed via the direct sum introduced in \Cref{appx:directsum}.

\begin{figure}[t]
{\small
  \[
  \begin{array}{c}
  {\hspace{-1em}
  \begin{array}{l@{\;\;\;}l@{\;}c@{\;}l @{\qquad} l@{\;\;\;}l@{\;}c@{\;}l @{\qquad} l@{\;\;\;}l@{\;}c@{\;}l @{\qquad} l@{\;\;\;}l@{\;\;}l}
  \text{Nat. Num} & m, n, j, k & \in & \mathbb{N}
&
\text{Real Number} & \theta, r & \in & {\mathbb{R}}
&
\text{Complex Number} & z & \in & {\mathbb{C}}
&
      \text{Variable} & x,y,f,g 
\end{array}
}
\\[0.3em]
  \begin{array}{l@{\quad}l@{\;\;}c@{\;\;}l@{}c@{\;\;\;}l} 
\text{Single Site Basis Vector in } \Hilb_{m} & \eta & ::= & {\displaystyle \ket{k}} && k\in[0,m)
\\
n\text{ Site Basis-ket State} & w & ::= &  {\displaystyle \Motimes_{k=0}^{n-1} \eta_{k} }
%\\[0.2em]
%\text{Single Particle Type With }$n$\text{ Spins} & t(n,m) & ::= &  {\bigotimes^{n}\textcolor{spec}{\mathpzc{H}^{m}}}
%\\[1em]
%\text{Single Particle State} & v & ::= & {\displaystyle{\sum_j} z_j\eta_j }
\\[0.5em]
\text{Quantum State Type} & \iota & ::= & t^{[\aleph]}(m) &\mid& \iota \ttimes \iota
\\[0.2em]
\text{Quantum State} & \psi & ::= & {\displaystyle {\sum_j} z_j w_j  } &\mid& \zero
    \end{array}
        \end{array}
  \]
}
\vspace*{-1.2em}
  \caption{\qsnd state structure for particles. A $t(m)$ typed basis vector $\ket{j}$ can have $j \in [0,m)$.  We abbreviate $z \cdot \Motimes_{k=0}^{0} \eta_{k} \equiv z\, \eta_0$, and $z_1\eta_1 \otimes z_2\eta_2\equiv (z_1 * z_2)\eta_1 \eta_2$. $[\aleph]$ means an opetional $\aleph$ flag. }
  \label{fig:data}
  \vspace*{-1em}
\end{figure}

\ignore{
\begin{figure}[t]
{\small
  \[
  \begin{array}{c}
  {\hspace{-1em}
  \begin{array}{l@{\;\;\;}l@{\;}c@{\;}l @{\qquad} l@{\;\;\;}l@{\;}c@{\;}l @{\qquad} l@{\;\;\;}l@{\;}c@{\;}l @{\qquad} l@{\;\;\;}l@{\;\;}l}
  \text{Nat. Num} & m, n, j, k & \in & \mathbb{N}
&
\text{Real Number} & r & \in & {\mathbb{R}}
&
\text{Complex Number} & z & \in & {\mathbb{C}}
&
      \text{Variable} & x,y,f,g 
\end{array}
}
\\[1.1em]
  \begin{array}{l@{\quad}l@{\;\;}c@{\;\;}l@{}c@{\;\;\;}l} 
\text{Single-site Computational Basis Vector in $\Hilb_{m}$} & \eta_k & ::= & {\displaystyle \ket{k}} && k\in[0,m)
\\[0.4em]
\text{$n$-site Computational Basis Vector} & w & ::= &  {\displaystyle \Motimes_{k=0}^{n-1} \eta_{k} }
%\\[0.2em]
%\text{Single Particle Type With }$n$\text{ Spins} & t(n,m) & ::= &  {\bigotimes^{n}\textcolor{spec}{\mathpzc{H}^{m}}}
%\\[1em]
%\text{Single Particle State} & v & ::= & {\displaystyle{\sum_j} z_j\eta_j }
\\[1.3em]

\text{Quantum State} & \psi & ::= & {\displaystyle {\sum_{j=1}^{m^n}} z_j w_j  } 
&\mid &\zero

\\[1.4 em]

\text{Quantum State Type} & \iota & ::= & t^{[\aleph]}(m) &\mid& \iota \ttimes \iota
    \end{array}
        \end{array}
  \]
}
\vspace*{-1.2em}
  \caption{\qsnd state structure.  
  A quantum state is a linear combination of computational basis vectors with complex amplitude $z_j$. $\zero$ symbolizes empty state.
  $t^{[\aleph]}(m)$ is a parameterized single-site type constructor,
  where $\aleph$ denotes the particle type, 
  $m$ denotes the dimension of the Hilbert space,
  and the square bracket "[]" means it is optional (it is omitted for identity operator). 
  The type of a state is composed of arbitrary number of single-site type constructor.
  }
  \label{fig:data}
  \vspace*{-1em}
\end{figure}
}

In describing quantum states, Dirac (bra-ket) notation \cite{Dirac1939} is commonly used.
We frenquently write a $\Hilb_m$ particle state as $z_0\ket{0} + ... + z_{m-1}\ket{m-1}$, where basis-ket vectors ($\eta$) $\ket{0} = \begin{psmallmatrix} 1 \\ 0 \\... \end{psmallmatrix}$ and $\ket{1} = \begin{psmallmatrix} 0 \\ 1 \\... \end{psmallmatrix}$, and so on. These vectors are \emph{computational basis-vectors} and $z_j\ket{j}$ is typically called a basis-ket. When more than one amplitudes ($z_j$) being non-zero, e.g., $z_j\ket{j} + z_k\ket{k} + z_i\ket{i}$ ($j$, $k$, and $i$ are distinct and $z_j$, $z_k$, and $z_i$ are non-zero), we can think of the particle being ``being in $j$, $k$, and $i$ at once,'' a.k.a. in a \emph{superposition} \cite{mike-and-ike}. In a qubit system, $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$ represents an equal superposition of $\ket{0}$ and $\ket{1}$. 
%In the quantum computer setting, a quantum qubit state $\psi$ \footnote{In quantum mechanics, $\ket{\psi}$ and $\bra{\psi}$ are used to express a quantum state and a conjugate transpose of a state. We use $\psi$ and $\sdag{\psi}$ in this paper to avoid confusion with basis-kets.} 
%
%We frequently write the qubit vector as $\alpha\ket{0} + \beta\ket{1}$ (the Dirac notation \cite{Dirac1939ANN}), where $\ket{0} = \begin{psmallmatrix} 1 \\ 0 \end{psmallmatrix}$ and $\ket{1} = \begin{psmallmatrix} 0 \\ 1 \end{psmallmatrix}$ are \emph{computational basis-kets}. When both $\alpha$ and $\beta$ are non-zero, we can think of the qubit being ``both 0 and 1 at once,'' a.k.a. in a \emph{superposition} \cite{mike-and-ike}, e.g., $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$ represents an equal superposition of $\ket{0}$ and $\ket{1}$.
Larger quantum values can be formed by composing smaller ones with the \emph{tensor product} ($\otimes$) from linear algebra, e.g., the two-qubit value $\ket{0} \otimes \ket{1}$ (also written as $\ket{0}\ket{1}$) corresponds to vector $\begin{psmallmatrix} 0 \\ 1 \\ 0 \\ 0 \end{psmallmatrix}$.
% 
However, many multi-particle values cannot be \emph{separated} and expressed as the tensor product of smaller values; such inseparable value states are called \emph{entangled},
e.g.\/ $\frac{1}{\sqrt{2}}(\ket{0}\ket{0} + \ket{1}\ket{1})$, known as a \emph{Bell pair} in a qubit system.

\Cref{fig:data} shows the quantum state syntax table used in \qsnd, which models the above typed Hilbert space based on \emph{computational basis-vectors and basis-kets}.
The quantum state syntax represents a conventional computational basis notation and naming convention used in the paper. It does not restrict the use of different forms of state representation, as any Hilbert space-based quantum state can be represented in the form shown in the figure.
%
In our system, we classify a $t^{[\aleph]}(m)$ type single particle basis vector state as the ket $\eta=\ket{k}$, with $k \in[0,m)$, referring to that the particle can be one ($k$) of the $m$ different basis-vector state. One can compose $n$ different particles together as a particle system basis-vector state as $w=\Motimes_{k=0}^{n-1} \eta_{k}$.
For example, two typed $t(3)$ particles can be in basis-vector states $\ket{2}$ and $\ket{1}$, we represent the whole basis-vector as $\ket{2} \otimes \ket{1}=\ket{2}\ket{1}$.
Here, the two kets both have the upper bound $3$.

In a quantum state, a typed $t(m)$ basis-ket state can be associated with a complex amplitude, as $z\ket{k}$.
We assume an $n$ particle basis-vector state as $w=\Motimes_{k=0}^{n-1} \eta_{k}$, which can be associated with amplitudes, e.g., $z_1\eta_1 \otimes z_2\eta_2$ can be abbreivated as $(z_1 * z_2)\eta_1 \eta_2$.
It is trivial that we can always associate the amplitude terms $z_j$ with a whole basis-vector term $w_j$.
In our formalism, we assume a quantum state has the canonical form as the summation formula $\psi = {\sum_j} z_j w_j$, of basis-ket states, to represent a quantum superposition state.
We include the zero vector $\zero$ in analyzing second quantization programs, discussed shortly below.

\subsection{Hamiltonian Simulation and Second Quantization}\label{sec:background2}

Quantum \emph{Hamiltonian simulation} involves implementing the operation $\eexp{\hat{H} r}$, denoted as $\eexp{r \hat{H}}$ in this paper for uniformity. on a quantum computer where $\hat{H}$ is the Hamiltonian (Hermitian $\hat{H} = \sdag{\hat{H}}$) of the simulated system. 
The unitary operation can be implemented as a quantum circuit program; the background information about unitary digital quantum circuits is in \Cref{sec:background3}.
A typical implementation is to perform Trotterization (explained shortly in \Cref{sec:sim-gates}), where we can decompose $\hat{H}$ into a weighted sum of an array of Hamiltonian terms $\hat{H} = \sum_{j} z_j P_j$. $z_j$ is the amplitude term, typically being a real number \footnote{Any Hermitian Hamiltonian can be rewritten in to a Pauli string form with only real number amplitudes; see \Cref{sec:compilecanonical}.}, and $P_j$ is a term that can be written as tensors of \emph{element operations}.
%
A typical selection of the element operations is the Pauli groups. In this case, we name such a tensor ($P_j$) as a \emph{Pauli string}.
For example,  for an $n$-site system, an $n$-site Pauli string is defined as $P_j = \sigma_n \otimes \sigma_{n-1} \otimes ... \otimes \sigma_1$, with $\sigma_k \in \{I, X, Y, Z\}$. Each $\sigma_k$ is applied to a qubit system with each site being $\Hilb_2$. 

\emph{Second Quantization} is a formalism to describe systems with varying numbers of particles. A second quantization program is still an Hamiltonian, with the element operations being application sequences of creators (\(\sdag{a}\)) and annihilators (\(a\)), as $\overline{\alpha} = \alpha_1 \circ ... \circ \alpha_j\circ ...$, with $\alpha_j\in\{a, \sdag{a}\}$ and $\circ$ being matrix multiplication. The intuition is to add or remove particles from a quantum state, respectively.
We name the tensors of $\overline{\alpha}$ to be \emph{tensor string}. In an $n$-site particle system, a tensor string $P_j$ could be $\overline{\alpha}_n \otimes \overline{\alpha}_{n-1} \otimes ... \otimes \overline{\alpha}_1$. 

In many case, an $n$-site Hamiltonian might contain an indexed syntactic sugar, such as $a(j) + \sdag{a}(j)$, expanded as $\textcolor{teal}{\Motimes_{k=0}^{j\sminus 1} I \otimes (a + \sdag{a}) \otimes \Motimes_{k=j\splus 1}^{n\sminus 1}I}$ in an $n$ particle system, i.e., a tensor string with the $j$-th position being the operation $a + \sdag{a}$ and the rests are identity operations. If there are more than two operations with the indexed sugar, we typically connect the two operations via function composition, e.g., $\sapp{\sdag{a}(j)}{ a(j\splus 1)}$, which can be expanded as follows. 

{\small
\begin{center}
$
\textcolor{teal}{\big(\Motimes_{k=0}^{j\sminus 1} I \otimes \sdag{a} \otimes \Motimes_{k=j\splus 1}^{n\sminus 1}I\big) \circ
\big(\Motimes_{k=0}^{j} I \otimes a \otimes \Motimes_{k=j\splus 2}^{n\sminus 1}I\big)}
=
\textcolor{teal}{\Motimes_{k=0}^{j\sminus 1} I \otimes \sdag{a} \otimes a \otimes \Motimes_{k=j\splus 2}^{n\sminus 1}I}
$
\end{center}
}

There are many interpretations of creators and annihilators in second quantization based on different particle types, which \qsnd classifies them in our type system.
The basic form is the creators and annihilators in \emph{a two-dimensional boson-like particle system}: the lowering $a$ and raising $\sdag{a}$ operations in ladder algebra, with the semantic rules below.
In this system, as shown above, applying a single creator $\sdag{a}$ (having the matrix representation 
$\begin{psmallmatrix}
0 & 0\\
1 & 0
\end{psmallmatrix}$) turning $\ket{0}$ to $\ket{1}$, but it eliminates $\ket{1}$ to be $\zero$,
while applying a single annihilator $a$ (having the matrix representation
$\begin{psmallmatrix}
0 & 1\\
0 & 0
\end{psmallmatrix}$) turning $\ket{1}$ to $\ket{0}$, but it eliminates $\ket{0}$ to be $\zero$.

{\small
\[\hspace{-0.2em}
\begin{array}{c}
\sdag{a}\ket{0}= \ket{1}
\qquad\qquad
\sdag{a}\ket{1}= \zero
\qquad\qquad
a\ket{1}= \ket{0}
\qquad\qquad
a\ket{0}= \zero
\\[0.3em]
\mapp{\sdag{a}}{a}\ket{1}=\ket{1}
\qquad\quad
\mapp{\sdag{a}}{a}\ket{0}=\zero
\qquad\quad
\mapp{a}{\sdag{a}}\ket{0}=\ket{0}
\qquad\quad
\mapp{a}{\sdag{a}}\ket{1}=\zero
\\[0.3em]
{\mapp{\sdag{a}}{a}}\otimes {\mapp{a}{\sdag{a}}}\ket{1}\ket{0}=\ket{1}\ket{0}
\qquad
{\mapp{\sdag{a}}{a}}\otimes {\mapp{a}{\sdag{a}}}\ket{b_1}\ket{b_2}=\zero\;\;\text{if}\;b_1\neq 1 \vee b_2 \neq 0
\end{array}
\]
}

We define the $\mathbb{0}$ and $\mathbb{1}$ operations in \Cref{sec:intro} by composing creators and annihilators,
i.e., $\mapp{\sdag{a}}{a}$, defining $\mathbb{1}$, preserves $\ket{1}$, and $\mapp{a}{\sdag{a}}$, defining $\mathbb{0}$, preserves $\ket{0}$, as shown in the second line above.
As an instance in a two qubit system, $\frac{1}{\sqrt{2}}(\ket{0}\ket{1} + \ket{1}\ket{0})$, applying $\mathbb{1}$ to the second site results the state $\frac{1}{\sqrt{2}}\ket{0}\ket{1}$ \footnote{This is the constraint semantics not the quantum dynamic unitary semantics, so operations are not necessarily unitary.}, by preserving $\ket{1}$ in the second site.
The composition effect can also deal with a composed state of multiple qubits, such as the third line above, with transitions below.

{\small
\begin{center}
$
\textcolor{teal}{{\mapp{\sdag{a}}{a}}\otimes {\mapp{a}{\sdag{a}}}\ket{1}\ket{0}}
=
\textcolor{teal}{{\mapp{\sdag{a}}{a}}\otimes {\mapp{a}{\sdag{a}}} (\ket{1} \otimes \ket{0})}
=
\textcolor{teal}{{\mapp{\sdag{a}}{a}}\ket{1}\otimes {\mapp{a}{\sdag{a}}} \ket{0}}
=\textcolor{teal}{\ket{1}\ket{0}}
$
\end{center}
}

We can see that Pauli strings are a special case of tensor strings, as one can construct Pauli strings by performing the above two-dimensional lowering and raising operations. The identity operation $I$ below is assumed to be two-dimensional.

{\small
\[
\begin{array}{l@{\qquad\quad}l@{\qquad\quad}l@{\qquad\quad}l}
I \triangleq  
\begin{bmatrix}
1 & 0\\
0 & 1
\end{bmatrix}
&
X \triangleq  
\begin{bmatrix}
0 & 1\\
1 & 0
\end{bmatrix}
&
Y \triangleq  
\begin{bmatrix}
0 & \sminus i\\
i & 0
\end{bmatrix}
&
Z \triangleq  
\begin{bmatrix}
1 & 0\\
0 & \sminus 1
\end{bmatrix}
\\[1em]
I = \sapp{a}{\sdag{a}} + \sapp{\sdag{a}}{a} = \mathbb{0} + \mathbb{1}
&
X = \sdag{a} + a
&
Y = i a - i \sdag{a}
&
Z = \sapp{a}{\sdag{a}} - \sapp{\sdag{a}}{a} =\mathbb{0} -  \mathbb{1}
\end{array}
\]
}

The second line above defines Pauli operations based on the two-dimensional lowering and raising operations above, with the matrix forms of the Pauli operations listed as the first line above.
Here, \(i\) is a complex amplitude value, and \(i a - i \sdag{a}\) is an abbreviation of \(\uapp{i}{a} + (\uapp{(\sminus i)}{\sdag{a}})\). 
Note that the meaning of Pauli groups in terms of second quantization differs from the gates in a quantum circuit, which provides a way of defining particle constraints by describing particle movements as spin rotations across \(X\), \(Y\), and \(Z\) bases.
%which provides a different view of particle movements in a Hamiltonian snapshot. Instead of describing electron occupation by creators and annihilators, Pauli groups describe particle movements as spin rotations across \(X\), \(Y\), and \(Z\) bases.
%\footnote{They are the bases in Lie Algebra \cite{Samelson1969NotesOL}. Intuitively, they enable rotations in three different axes.}. 

%Measurement in quantum mechanics projects the quantum state onto an eigenstate of the observable being measured. For a qubit in state \(|\psi\rangle = \alpha|0\rangle + \beta|1\rangle\), a measurement in the computational basis yields \(|0\rangle\) with probability \(|\alpha|^2\) and \(|1\rangle\) with probability \(|\beta|^2\).
% A special, non-unitary \emph{measurement} operation is used to extract classical information from a quantum state, typically when a computation completes. Measurement collapses the state to one of the basis states with a probability related to the state's amplitudes. For example, measuring $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$ will collapse the state to $\ket{0}$ with probability $\frac{1}{2}$ and likewise for $\ket{1}$, returning classical values 0 or 1, respectively. In all the programs discussed in this paper, we leave the final measurement operation implicit.
 %A \emph{measurement} operation extracts classical information from a quantum value. It collapses the value to a basis state with a probability related to the value's amplitudes (\emph{measurement probability}), e.g., measuring $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$ collapses the value to $\ket{0}$ with probability $\frac{1}{2}$,  and likewise for $\ket{1}$, returning classical value $0$ or $1$, respectively. 
%A more general form of quantum measurement is \emph{partial measurement}, which measures a subset of qubits in a qubit array;
% 
%such operations often have simultaneity effects due to entanglement, \ie{} in a Bell pair $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$,
%measuring one qubit guarantees the same outcome for the other --- if the first bit is measured as $0$, the second bit is too.

\subsection{QBlue: Second Quantization Language as Energy Constraint Programming}\label{sec:overview2}

The \qsnd language is based on second quantization. We first examine QBlue's programmability for directing users to write energy-constrained programs, mainly to answer how scientific computation users think of Hamiltonian programs.
Recall that the Hamiltonian constraint for $K$-clique finding is  $\textcolor{teal}{\sum_{j\neq m} (1-E(j,m)) * \sapp{\mathbb{1}(j)}{\mathbb{1}(m)}}$, where we search all the $k$-subgraphs and add penalties for pairs of vertices $j$ and $m$ in a subgraph that has no edge. If we compute the Hamiltonian energy value for a subgraph to be $0$, the subgraph is a clique. Such constraint programming can be done in adiabatic quantum computing (AQC).

Quantum particle system Hamiltonian essentially adopts these kinds of Hamiltonian constraint concepts.
We first show a Hubbard Model example \footnote{This is a simplified version, and a full version is in \Cref{sec:hubbard}.}, used to describe the tunnelling of quantum particles from one site to another by viewing sites as a lattice graph.
%The lattice graph and site concept is essentially a generalization of the quantum circuit diagram in \Cref{sec:background3},
%in the sense that each qubit is a site, operations in each circuit line represents a sequence of operation applying to the site, and multi-qubit opertions represent interactions across different sites. Defining Hamiltonian constraints based on the generalized lattice graph and site concept provides additional freedom for users to restrict how sites can communicate, e.g., we can restrict that some circuit lines in \Cref{sec:background3} are not capable of communication.
The Hamiltonian below operates on sites holding fermions, described by a two-dimensional Hilbert space ($\Hilb_2$).

{\small
\[
\hat{H}_T = \sminus z_t \sum_{j} 
\left(\sapp{\stype{\sdag{a}(j)}{t^{\aleph}(2)}}{ \stype{a(j\splus 1)}{{t^{\aleph}(2)}}} + \sapp{\stype{\sdag{a}(j\splus 1)}{{t^{\aleph}(2)}}}{ \stype{a(j)}{{t^{\aleph}(2)}}}\right) + z_u \sum_{j}  \sapp{\stype{\mathbb{1}(j)}{{t^{\aleph}(2)}}}{\stype{\mathbb{1}(j\splus 1)}{{t^{\aleph}(2)}}}
\tag{2.3.1}\label{eq:hubbard}
\]
}

Before examining the program behavior, we first identify three layers of Hamiltonian program semantics for any Hamiltonian system below.

\begin{itemize}
\item \emph{Constraint Semantics} refers to a Hamiltonian (a Hermitian matrix), applicable to a state; such semantics describes the constraint among different particle sites, and the operations represent quantum constraints of the user's intention for a system.
\item \emph{Dynamic Semantics} refers to Hamiltonian simulation ($\eexp{r{\hat{H}}}$), where we learn about the state at time $r$, as $\psi(r)$, by simulating the Hamiltonian $\hat{H}$ on the initial state $\psi(0)$, as $\eexp{r{\hat{H}}}\psi(0)$; such simulation produces a unitary implementable in quantum computers.
\item \emph{Application Semantics} refers to finding the a \emph{minimized energy state} $\psi_{min}$ minimizing the constraints defined in $\hat{H}$, defined as $\cn{min}(\hat{H})$.
\end{itemize}

This paper does not formalize application semantics, but we show an example computation via the AQC method in \Cref{sec:cases}.
%The second layer is the Hamiltonian dynamic semantics in this paper, defined by the Hamiltonian simulation ($\eexp{\sapp{\hat{H}}{t}}$), referring to that we learn about the state at time $t$, as $\psi(t)$, by simulating the Hamiltonian $\hat{H}$ on the initial state $\psi(0)$.
%The third layer is the application semantics, defined by $\cn{min}(\hat{H})$, computing out a \emph{minimized energy state} $\psi_{min}$ minimizing the constraints defined in $\hat{H}$.
%We show a way of computing the minimized energy state via adiabatic quantum computation method in \Cref{sec:cases}.

We examine the constraint level program behavior of Hamiltonian programs. The Hubbard model program is similar to many other Hamiltonian constraint programs \cite{Lucas_2014,10.21468/SciPostPhys.8.2.021}, where they can be partitioned into an initial Hamiltonian and a final Hamiltonian, connected by a sum operation. In this paper, we classify initial Hamiltonians as \emph{motion Hamiltonians} $\hat{H}_{m}$ and final Hamiltonians as \emph{problem Hamiltonians} $\hat{H}_p$, where the names indicate the constraint behavior.

If we view the ket numbers in each site as the number of particles occupying the site,
motion Hamiltonians define the constraints for the potential particle movement in different sites.
The motion Hamiltonian $\textcolor{teal}{\sminus z_t \sum_{j} (\sapp{\sdag{a}(j)}{ a(j\splus 1)} + \sapp{\sdag{a}(j\splus 1)}{ a(j)})}$ indicates that the appearance of a particle in the $j$-th site ($\sdag{a}(j)$) results in the particle disappearance in the $j\splus 1$-th site, and vice versa.


\begin{wrapfigure}{r}{3.3cm}
%\vspace*{-2.5em}
  \includegraphics[width=0.25\textwidth]{demo.pdf}
%\vspace*{-0.5em}
  \caption{Analogy}
%\vspace*{-1em}
\label{fig:analogy}
\end{wrapfigure}

Another common motion Hamiltonian is $\textcolor{teal}{\sum_{\cn{j}=0}^n(\sdag{a}(j)+a(j))}$ in a $t(2)$ system, e.g., applying Pauli $X$ ($X=\sdag{a}+a$) to every $j$-th site. 
An $n$ qubit uniform superposition state $\textcolor{teal}{\frac{1}{\sqrt{2}}\sum_{k=0}^{2^n} \ket{k}}$ is the eigenstate of the motion Hamiltonian.
A utility of the Hamiltonian is in the D-Wave-based AQC system \cite{dwave2025}. Users start with the above superposition state, with the setting of the above motion Hamiltonian, and apply the AQC procedure to approximate the desired solution.
To understand the program behavior of a motion Hamiltonian, its Hamiltonian simulation is as if there is an assembly line, and each worker is dealing with a single basis-ket in the superposition state.
As demonstrated in the analogy in \Cref{fig:analogy}, Alice and Bob are two workers dealing with two basis-kets.
Applying an operation $\textcolor{teal}{\sdag{a}(j)+a(j)}$ on the first qubit means that we make a product shift of the assembly line based on the first position of each basis-ket, so that Alice and Bob swap the basis-kets they were dealing.
Different initial superposition states might require different motion Hamiltonians, i.e., $\textcolor{teal}{\sum_{j} (\sapp{\sdag{a}(j)}{ a(j\splus 1)} + \sapp{\sdag{a}(j\splus 1)}{ a(j)})}$ is the motion Hamiltonian for the $k$-hamming weight initial superposition state, see \Cref{sec:cases}.

Problem Hamiltonians, e.g., the $\textcolor{teal}{\hat{H}_p = z_u \sum_{j}  \mathbb{1}(j) \circ \mathbb{1}(j\splus 1)}$ in $\hat{H}_T$ above, represent the particle properties in a problem. $\hat{H}_p$ can be rewritten as  $\textcolor{teal}{z_u \sum_{j} (\mapp{\sdag{a}(j)}{a(j)}) \circ (\mapp{\sdag{a}(j\splus 1)}{ a(j\splus 1)})}$.
In defining a particle system constraint, users typically think of the occupied number of particles in a site, as a way to express their constraint, i.e., they express the constraints as a certain basis-vector in a site, e.g., $\ket{0}$ represents a site is empty or $\ket{1}$ represents a site is occupied with a particle.
However, the quantum superposition state is not directly observable. Instead of manipulating the ket states, we use second quantization operations represent the constarints for desired ket states, e.g., we use $\mathbb{1}$ and $\mathbb{0}$ to respectively constraint $\ket{1}$ and $\ket{0}$ in a $t(2)$ typed system, because $\mathbb{1}$ preserves $\ket{1}$ but removes $\ket{0}$ and $\mathbb{0}$ preserves $\ket{0}$ but removes the $\ket{1}$.
For representing a $\ket{k}$ state, one can easily define a operation $\mathbb{K}$, by rewriting $k$ in the binary format $d_k$ and then define $\mathbb{K}$ as a tensor string with the $j$-th element operation being $\mathbb{1}$ and $\mathbb{0}$ representing $d_k[j]$.
For example, the $\hat{H}_p$ above has the constraint semantics that if two adjacent sites show both $\ket{1}$, we apply a penalty ($z_u$) constraint to the system, and the simulation of the system should reach a state minimizing energy penalties.
%Particularly, the problem Hamiltonian in the Hubbard model suggests that we want to add a penalty $z_u$, if two adjacent sites having occupied particles ($\ket{1}$).
%In the above Hubbard model program, the term $\mapp{\sdag{a}(j)}{ \mapp{a(j)}{\mapp{\sdag{a}(j\splus 1)}{ a(j\splus 1)}}}$ means we applying two $\mathbb{1}$ ($\mapp{\sdag{a}}{a}$) operations to two adjacent sites ($j$ and $j\splus 1$), referring to that we impose a penalty constraint if two adjacent sites are occupied by two fermions.

\subsection{The QBlue Compiler and Optimization Algorithms}\label{sec:sim-gates}

%\liyi{This section overviews the compiler with figures, and an example.}
Hamiltonians represent constraints that users intend to do, which are not directly compilable.
A typical Hamiltonian usage is to compile its Hamiltonian simulation \cite{Tacchino_2019,Li_2022,cao2024marqsimreconcilingdeterminismrandomness,10.1145/3503222.3507715}, the Hamiltonian's dynamic semantics, to quantum computers for execution. We dicuss below the key \qsnd features to compile Hamiltonian simulation.

\noindent{\textbf{\emph{Adding Types in \qsnd.}}}
%
Without specifying the two-dimensional fermion state indication, e.g., the mark \textcolor{spec}{blue} type information, one cannot determine what kind of systems the Hubbard model Hamiltonian $\hat{H}_T$ constraint describes, e.g., the same program can represent a boson system \cite{peng2023quantum}.
To constrain the system for fermions, \qsnd types each site as $t^{\aleph}(2)$, referring to a two-dimensional fermion state.
\qsnd also classifies a qubit system above having $t(2)$ typed sites, as a qubit and a $t(2)$ typed boson behave the same.
The types can help classify different sites in \qsnd and permit the interactions of different quantum particles.
We permit other particle types; see \Cref{sec:formal}.
The typing is useful when transforming a particle system to another, often in analyzing different particle systems.
For example, when compiling a two particle $t(m)$ typed system $\hat{H}$, with typing $t(m) \otimes t(m)$, to a qubit system with each site being $t(2)$ type,
we notice that a basis-vector state $j \in [0,m)$ in a particle, whose binary form can be represented by a bitstring with the length $N=\ulcorner \log(m) \urcorner$.
The above two particle system can be compiled to a $\Motimes^{2*N}$ typed qubit system, each qubit is typed as $t(2)$. Considering the two particle system Hamiltonian simulation as a function $\Motimes^2 t(m) \to \Motimes^2 t(m)$, the compilation is typed as the high-order function below.

{
\begin{center}
$
\textcolor{spec}{(\Motimes^2 t(m) \to \Motimes^2 t(m)) \to (\Motimes^{2*N} t(2) \to \Motimes^{2*N} t(2))}
$
\end{center}
}

%Our type construct, $t(n,m)$, also crystallizes the spin concept in our second quantization formalism.
%Recall in \Cref{fig:data} that the $t(n,m)$ type essentially represents tensors of Hilbert space ${\bigotimes^{n}{\mathpzc{H}^{m}}}$ for describing each particle site, and each Hilbert space describes a spin.
%One can think of the spins as if we have $n$ different counters in a particle site, and applying an operation with a spin flag refers to applying it to the right counter.
%To understand the concept clearly, let's focus on the $t(2,2)$ typed particle case, which has two possible spins.
%Here, \(\ket{1}_0\ket{0}_1\) (written as \(\ket{\uparrow}\) in some literature) means that a particle site contains a spin-up ($\uparrow$) electron, while \(\ket{0}_0\ket{1}_1\) (traditionally written as \(\ket{\downarrow}\)) refers to a particle site containing a spin-down ($\downarrow$) electron. Obviously, applying a annihilator $a_{0}$ to \(\ket{1}_0\ket{0}_1\) results in \(\ket{0}_0\ket{0}_1\) (traditionally written as \(\ket{0}\)) and applying a creator $a_{1}$ to the above state results in \(\ket{1}_0\ket{1}_1\) (traditionally written as \(\ket{\uparrow\downarrow}\)).
%The \qsnd type information clarifies the spin behaviors, as some systems \cite{10.1145/3632923} misinterpreted spin-up and down as qubits $\ket{0}$ and $\ket{1}$ without proper compilation.
%As we show here, they are not identical.

\noindent{\textbf{\emph{An End-to-End Compilation.}}}
Previous Hamiltonian simulation compilation works are either example-based \cite{Li_2022,Tacchino_2019} without formalism, or focus on specific subroutines, such as Trotterizations \cite{cao2024marqsimreconcilingdeterminismrandomness,10.1145/3503222.3507715}.
\qsnd intends to provide the first end-to-end compilation formalism for compiling Hamiltonian simulation for any second quantization Hamiltonian programs to quantum circuits, both digital and analog-based.
%Finding the right target machine Hamiltonian to simulate a gate, i.e., gate synthesis, is usually referred to as control pulse level quantum programming \cite{Li_2022,Tacchino_2019} as control pulses can theoretically be described as \emph{target machine Hamiltonians}, and previous work \cite{10.1145/3632923} has discovered the advantage of compiling system Hamiltonians directly to target machine Hamiltonians by bypassing the series of simulations of individual gates.
To see how our compiler works, we simulate a simple $t(2)$ typed Ising model system $\hat{H}_{I1}$ below, describing phase transition and quantum magnetism behaviors in insulating magnetic systems.

{\small
\[
\begin{array}{ll}
&z_h \sum_j \big(\stype{\sdag{a}(j)}{t(2)} + \stype{a(j)}{t(2)} \big) + \sum_{j} {\big(\stype{\mathbb{0}(j)}{t(2)} - \stype{\mathbb{1}(j)}{t(2)}\big)}\circ {\big(\stype{\mathbb{0}(j\splus 1)}{t(2)}-\stype{\mathbb{1}(j\splus 1)}{t(2)}\big)}
\\[0.3em]
\looongrightarrow& z_h \sum_j X(j) + \sum_{j} {Z(j)}\circ{Z(j\splus 1)}
\end{array}
 \tag{2.4.1}\label{eq:ising}
\]
}


\begin{figure*}[t]
{\small
\begin{tabular}{c@{$\;\;=\;\;$}c}
\begin{minipage}{0.22\textwidth}
$
\eexp{\frac{r}{n}{\sapp{Z(j)}{Z(j\splus 1)}}}
$
\end{minipage}
&
\begin{minipage}{0.3\textwidth}
{
  \Qcircuit @C=0.5em @R=0.5em {
    \lstick{} & & \ctrl{1}       & \qw  & \ctrl{1}      &\qw\\
    \lstick{} & & \targ         & \gate{\cn{Rz}(2\frac{r}{n})}       & \targ    & \qw 
    }
}   
\end{minipage}
\end{tabular}
\hspace{1em}
\begin{minipage}{0.41\textwidth}
{\small
$
ZZ(\theta)=
\begin{psmallmatrix}
\cn{exp}(\sminus i\frac{\theta}{2}) & 0 & 0 & 0\\
 0 & \cn{exp}(i\frac{\theta}{2}) & 0 & 0\\
 0 & 0 & \cn{exp}(i\frac{\theta}{2}) & 0\\
 0 & 0 & 0 & \cn{exp}(\sminus i\frac{\theta}{2})
\end{psmallmatrix}
$
}
  \end{minipage}
}
\vspace*{-0.8em}
\caption{Circuit decomposition and unitary for $ZZ$ Interaction. The left circuit applies on $j$ and $j\splus 1$ qubits.}
\label{fig:zz-inter}
\vspace*{-1.2em}
\end{figure*}

The term in $\hat{H}_{I1}$, $z_h \sum_j \sdag{a}(j) + a(j)$, is the motion Hamiltonian constraining potential movements, and the second sum term is the problem Hamiltonian constraining the energy penalties. Suppose two adjacent sites have the same kets (both $\mathbb{0}$ or $\mathbb{1}$). In that case, there is a positive energy penalty, while if the two sites have opposite ket states (having one $\mathbb{0}$ and $\mathbb{1}$), there is a negative energy penalty, a.k.a., an incentive. Essentially, the problem Hamiltonian constrains that two adjacent sites describe magnetic forces.

To compile the Hamiltonian simulation $\eexp{r \hat{H}_{I1}}$ with respect to a time $r$ (in \qsnd, we typically write $r$ as amplitudes of Pauli operators in $\hat{H}_{I1}$), we first perform particle transformation (\Cref{sec:transformation}) to transform the system to a Pauli-based Hamiltonian, a.k.a., a sum of Pauli strings, as the right above. The main step in compiling the Pauli-based Hamiltonian simulation is Trotterization, a technique to split $\hat{H}_{I1}$ into small Hamiltonians, and perform Hamiltonian simulation for the smaller Hamiltonians in sequence to approximate $\eexp{r \hat{H}_{I1}}$.
In the above example, Trotterization produces a sequence of $\eexp{\frac{r}{n} {Z(j)}\circ{Z(j\splus 1)}}$ and $\eexp{\frac{r}{n} X(j)}$ operations (the sequence length is related to $n$). If $n$ is large enough, the operation sequence is a good approximation to $\eexp{r \hat{H}_{I1}}$.
The $\eexp{\frac{r}{n} X(j)}$ operation produces a \cn{Rx} gate (\Cref{sec:decompose}), while $\eexp{ \frac{r}{n} {Z(j)}\circ{Z(j\splus 1)}}$ produces a digital circuit as the left in \Cref{fig:zz-inter}, performing two controlled-not gates and an $\cn{Rz}(2\frac{r}{n})$ gate in the middle for the $j$-th and $j\splus 1$-th qubits,
i.e., $\cn{Rz}(\theta)$ is an $z$-axis phase rotation gate, rotating $\theta$ angle.

There is also analog-based compilation, which compiles Hamiltonian simulations to target machine Hamiltonians by viewing quantum computers as Hamiltonian simulators.
For example, IBM provides a direct programming support for $ZZ$ interaction gate shown as the right in \Cref{fig:zz-inter}; the special gate essentially simulates the target machine Hamiltonian $\sapp{Z(j)}{Z(j\splus 1)}$ in a much more effective way than the above digital circuit gate decomposition step.

\ignore{
In summary, these foundational concepts of quantum mechanics—quantum states, operators, the Schrödinger equation, and Hilbert spaces—are crucial for understanding and developing quantum computing. 




%Circuit-based quantum computation can also be generalized and viewed as a quantum simulation procedure based on the Schrödinger equation, explained shortly below.


%\myparagraph{Hamiltonian-based Quantum Applications}
%
%Hamiltonian is a Hermitian matrix \(\hat{H}\), where an operator is Hermitian if it equals its own conjugate transpose, $\hat{H} = \sdag{\hat{H}}$.

%\liyi{In the above, we need to use the same symbol. If Hamiltonian is H, then keep using H. In addition, there is no need to distinguish Hamiltonian vs Hermitian in CS, because they are not going to learn the difference. Just think of them as the same. We are not trying to teach them the entire quantum mechanics.}

%\liyi{I think below is unnecessary to relate to observables. I do not think people will understand observable, and they should not need to learn about observable.}
%Hermitian operators correspond to observables, quantities that can be measured. Their eigenvalues are real numbers, and their eigenvectors form an orthonormal basis for the Hilbert space. Examples of Hermitian operators include:


%From the perspective of quantum mechanics, quantum computation can be viewed as a quantum simulation procedure based on the Schrödinger equation, involving unitary operations and quantum states. In this context, a quantum unitary operation may be defined as an exponential of a Hamiltonian.


%The circuit in \Cref{fig:background-circuit-examplea} uses $n$ qubits and applies $n$ gates: a \emph{Hadamard} (\coqe{H}) gate and $n-1$ \emph{controlled-not} (\coqe{CNOT}) gates.
%Applying a gate to a quantum value \emph{evolves} it.
% 
%Its traditional semantics is expressed by multiplying the value's vector form by the
%gate's corresponding matrix representation: $n$-qubit gates are $2^n$-by-$2^n$
%matrices.




In quantum mechanics, when describing a quantum state, its basis element is typically not a qubit, but a particle site.
A quantum state is represented by a vector in a Hilbert space, which is a complete vector space with an inner product. For a single qubit, the state is described as:

\[
|\psi\rangle = \alpha|0\rangle + \beta|1\rangle
\]

where \(|0\rangle\) and \(|1\rangle\) are basis states, and \(\alpha\) and \(\beta\) are complex coefficients such that \(|\alpha|^2 + |\beta|^2 = 1\). This representation is known as Dirac notation, or bra-ket notation \cite{dirac1939}. In this context, we will consider only normalized states, which satisfy \(\langle \psi | \psi \rangle = 1\).

%\liyi{below is subject to change. No reviewer in POPL will understand any of this. The problem is that they should not try hard to understand this. This is background, and the purpose is to make them comfortably accept these. }
\section*{Hilbert Spaces and Tensor Products}

The Hilbert space of a single qubit is a two-dimensional complex vector space. For multiple qubits, the total Hilbert space is the tensor product of the individual qubit spaces. For two qubits:

\[
\Hilb = \Hilb_1 \otimes \Hilb _2
\]

where \(\Hilb_1\) and \(\Hilb_2\) are the Hilbert spaces of the individual qubits, each of dimension 2. The combined space has dimension \(2^2 = 4\). For \(n\) qubits, the total Hilbert space has dimension \(2^n\).

\section*{Operators}

Operators act on quantum states to produce new states or to extract information about the system. Key types of operators in quantum mechanics include Hermitian and unitary operators.

\subsection*{Hermitian Operators}

An operator \(\hat{A}\) is Hermitian if it equals its own conjugate transpose:

\[
\hat{A} = \hat{A}^\dagger
\]

Hermitian operators correspond to observables, quantities that can be measured. Their eigenvalues are real numbers, and their eigenvectors form an orthonormal basis for the Hilbert space. Examples of Hermitian operators include:

\liyi{bad example. no CS people will understand.}
\begin{itemize}
    \item \textbf{Spin operator (\(\hat{S}_z\))}: Measures the spin of a particle along the z-axis.
    \item \textbf{Hamiltonian (\(\hat{H}\))}: Represents the total energy of the system.
\end{itemize}

The expectation value of a Hermitian operator \(\hat{A}\) in a state \(|\psi\rangle\) is given by:

\[
\langle \hat{A} \rangle = \langle \psi | \hat{A} | \psi \rangle
\]

This represents the average measured result of the physical variable corresponding to \(\hat{A}\) when the system is in state \(|\psi\rangle\).

\subsection*{Unitary Operators}

An operator \(\hat{U}\) is unitary if it satisfies:

\[
\hat{U}^\dagger \hat{U} = \hat{U} \hat{U}^\dagger = \hat{I}
\]

Unitary operators preserve the inner product and hence the norm of quantum states. They are used to describe the evolution of isolated quantum systems and perform quantum gates in quantum computing. Notably, the exponential of a Hermitian operator \(\hat{A}\) is unitary:

\[
\hat{U} = e^{i\hat{A}}
\]

Examples of unitary operators include:

\begin{itemize}
    \item \textbf{Rotation operator (\(\hat{R}(\theta)\))}: Rotates the state vector in a plane by an angle \(\theta\).
    \item \textbf{Pauli-X gate}: Acts like a classical NOT gate, flipping the state \(|0\rangle\) to \(|1\rangle\) and vice versa.
    \item \textbf{Hadamard gate}: Creates superposition by transforming \(|0\rangle\) into \(\frac{1}{\sqrt{2}}(|0\rangle + |1\rangle)\) and \(|1\rangle\) into \(\frac{1}{\sqrt{2}}(|0\rangle - |1\rangle)\).
\end{itemize}

\section*{The Schrödinger Equation}

The dynamics of a quantum system are governed by the Schrödinger equation.

\subsection*{Time-Independent Schrödinger Equation}

\[
\hat{H}|\psi\rangle = E|\psi\rangle
\]

where \(\hat{H}\) is the Hamiltonian, \(|\psi\rangle\) is an eigenstate, and \(E\) is the energy eigenvalue. The ground state corresponds to the lowest energy eigenvalue, while excited states have higher energies.

\subsection*{Variational Principle}

To find the exact ground state energy \(E_0\), one can use the variational principle. For a normalized state \(|\phi\rangle\), the expectation value of the Hamiltonian over all possible states \(|\psi\rangle\) is minimized:

\[
E_0 = \min_{|\psi\rangle} \langle \psi|\hat{H}|\psi\rangle
\]

By minimizing this expectation value over all possible normalized states, the exact ground state can be obtained.

\subsection*{Time-Dependent Schrödinger Equation}

\[
i \frac{\partial}{\partial t} |\psi(t)\rangle = \hat{H}|\psi(t)\rangle
\]

where \(t\) is the time variable. Its solution involves the propagator \(e^{-i\hat{H}t}\), which evolves the state from an initial state \(|\psi(0)\rangle\):

\[
|\psi(t)\rangle = e^{-i\hat{H}t}|\psi(0)\rangle
\]

\begin{comment}
\nonindent\textbf{\textit{Quantum Mechanics}}

Quantum mechanics is the branch of physics that describes the behavior of particles on the atomic and subatomic scale. A fundamental task in quantum mechanics is quantization, which involves transitioning from classical to quantum descriptions of physical systems. This process is essential for understanding how particles, such as electrons and photons, exhibit both wave-like and particle-like properties.

\subsection*{Quantum States}

A quantum state is a complete description of a quantum system, represented mathematically by a vector in a complex Hilbert space. The state of a quantum system is typically denoted by $\ket{\psi}$, known as a ket vector, which encapsulates all information about the system.

In general, a quantum state can be expressed as a superposition of basis states $\{\ket{\phi_i}\}$ of the Hilbert space:
\[
\ket{\psi} = \sum_i \alpha_i \ket{\phi_i}
\]
where $\alpha_i$ are complex coefficients, and $\sum_i |\alpha_i|^2 = 1$. The basis states $\{\ket{\phi_i}\}$ form an orthonormal basis, meaning $\langle \phi_i | \phi_j \rangle = \delta_{ij}$, where $\delta_{ij}$ is the Kronecker delta.

\subsection*{Physical Observables}

In quantum mechanics, physical quantities such as energy, momentum, spin, and magnetization are represented by operators acting on the quantum state vectors. These operators are Hermitian, ensuring that their eigenvalues, which correspond to the measurable values, are real numbers.

\subsubsection*{Hamiltonian}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

The Hamiltonian operator $\hat{H}$ represents the total energy of the system, including both kinetic and potential energy components. It governs the time evolution of the quantum state via the Schrödinger equation.

\paragraph*{Time-Dependent Schrödinger Equation:}
\[
i\hbar \frac{\partial}{\partial t} \ket{\psi(t)} = \hat{H} \ket{\psi(t)}
\]
For an initial state $\ket{\psi(0)}$, the time-evolved state $\ket{\psi(t)}$ can be expressed as:
\[
\ket{\psi(t)} = \exp\left(-\frac{i\hat{H} t}{\hbar}\right) \ket{\psi(0)}
\]

\paragraph*{Time-Independent Schrödinger Equation:}
\[
\hat{H} \ket{\psi} = E \ket{\psi}
\]
where $E$ represents the energy eigenvalue of the state $\ket{\psi}$.

\subsubsection*{Other Physical Observables}

\paragraph*{Spin:} The spin of a particle, such as an electron, is an intrinsic form of angular momentum. The spin operator $\hat{S}$ has components $\hat{S}_x$, $\hat{S}_y$, and $\hat{S}_z$, corresponding to measurements along different axes. For a spin-$\frac{1}{2}$ particle, the spin states are typically denoted as spin-up ($\ket{\uparrow}$) and spin-down ($\ket{\downarrow}$).

\paragraph*{Magnetization:} The magnetization of a material can be related to the collective spin states of its constituent particles. The magnetization operator can be represented as a sum of individual spin operators.

The expectation value of an observable $\hat{A}$ in a normalized state $\ket{\psi}$ is given by:
\[
\langle \hat{A} \rangle = \bra{\psi} \hat{A} \ket{\psi}
\]

\subsection*{Variational Principle}

The variational principle is a method used to approximate the ground state energy and corresponding wavefunction of a quantum system. According to this principle, for a given trial wavefunction $\ket{\phi}$, the expectation value of the Hamiltonian provides an upper bound to the ground state energy and as a result,

\[
E_0 = \min_{\ket{\phi}} \frac{\bra{\phi} \hat{H} \ket{\phi}}{\braket{\phi|\phi}}
\]

To find the best approximation to the ground state energy, one minimizes the expectation value of the Hamiltonian with respect to the parameters of the trial wavefunction. In the above, $\ket{\phi}$ may or may not be normalized. If $\ket{\phi}$ is normalized, then $\braket{\phi|\phi} = 1$, and the expression simplifies to:
\[
E_0 \leq \bra{\phi} \hat{H} \ket{\phi}
\]

\subsection*{Second Quantization}

Second quantization is a formalism that extends the principles of quantization to systems with multiple particles. It introduces the concept of creation and annihilation operators, which respectively add or remove particles from specific quantum states. This approach is particularly useful for describing systems where the number of particles can change, such as in quantum field theory. It is important to note that "second quantization" is simply another representation among many, and there is no actual "second quantization" process on top of the initial one.

In second quantization, particles are treated as indistinguishable, and their possible states are represented by occupation numbers, which indicate how many particles occupy each state. Each particle state can be described using a basis in an $n$-dimensional Hilbert space. The creation operator raises the occupation number of a state, while the annihilation operator lowers it. These operators are fundamental in describing interactions and dynamics in many-particle systems.

\subsection*{Examples}

\subsubsection*{Single Spin States}

Consider the quantum states of a spin-$\frac{1}{2}$ particle, such as an electron. These particles can exist in one of two spin states: spin-up ($\ket{\uparrow}$) or spin-down ($\ket{\downarrow}$). These states can be represented as two-dimensional vectors:
\[
\ket{\uparrow} = \begin{pmatrix} 1 \\ 0 \end{pmatrix}, \quad \ket{\downarrow} = \begin{pmatrix} 0 \\ 1 \end{pmatrix}
\]
A general spin state can be written as a superposition of these basis states:
\[
\ket{\psi} = \alpha \ket{\uparrow} + \beta \ket{\downarrow}
\]
where $\alpha$ and $\beta$ are complex numbers such that $|\alpha|^2 + |\beta|^2 = 1$.

\subsubsection*{Tensor Products}

Quantum systems with multiple particles can be described using tensor products of individual particle states. For example, consider a system of two spin-$\frac{1}{2}$ particles. The combined quantum state of the system can be represented as a tensor product of the states of each particle.

If the first particle is in state $\ket{\psi_1} = \alpha_1 \ket{\uparrow} + \beta_1 \ket{\downarrow}$ and the second particle is in state $\ket{\psi_2} = \alpha_2 \ket{\uparrow} + \beta_2 \ket{\downarrow}$, the combined state of the two-particle system is:
\[
\ket{\psi_{12}} = \ket{\psi_1} \otimes \ket{\psi_2} = (\alpha_1 \ket{\uparrow} + \beta_1 \ket{\downarrow}) \otimes (\alpha_2 \ket{\uparrow} + \beta_2 \ket{\downarrow})
\]

Expanding this tensor product, we get:
\[
\ket{\psi_{12}} = \alpha_1 \alpha_2 \ket{\uparrow\uparrow} + \alpha_1 \beta_2 \ket{\uparrow\downarrow} + \beta_1 \alpha_2 \ket{\downarrow\uparrow} + \beta_1 \beta_2 \ket{\downarrow\downarrow}
\]
where $\ket{\uparrow\uparrow}$, $\ket{\uparrow\downarrow}$, $\ket{\downarrow\uparrow}$, and $\ket{\downarrow\downarrow}$ are the basis states for the two-particle system.

\subsubsection*{Entanglement}

Some multi-particle states cannot be factored into tensor products of individual particle states. These inseparable states are known as entangled states. An example of an entangled state is the Bell state (or Bell pair):
\[
\ket{\Phi^+} = \frac{1}{\sqrt{2}} (\ket{\uparrow\uparrow} + \ket{\downarrow\downarrow})
\]
This state cannot be written as a tensor product of two single-particle states, indicating that the particles are entangled. In an entangled state, the measurement outcomes of one particle are correlated with those of the other particle, no matter how far apart the particles are.

These examples highlight the versatility of quantum states and the utility of tensor products in describing complex quantum systems, illustrating key concepts in quantum mechanics and second quantization.

\subsection*{Quantum Measurement} 

A \emph{measurement} operation extracts classical information from a quantum state. It collapses the state to one of its basis states with a probability related to the state's amplitudes (\emph{measurement probability}). For example, measuring the state \(\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})\) collapses the state to \(\ket{0}\) with probability \(\frac{1}{2}\), and to \(\ket{1}\) with the same probability, returning the classical value 0 or 1, respectively. 

A more general form of quantum measurement is \emph{partial measurement} can be examplified by a measurement of a subset of qubits in a multi-qubit system. These operations often have simultaneous effects due to entanglement. For instance, in the Bell state \(\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})\), measuring one qubit determines the outcome of the other. If the first qubit is measured as 0, the second qubit is also 0, and similarly for 1.

In addition to the standard measurement, general projection measurements involve projecting a quantum state onto a subspace defined by a projection operator. Given a quantum state \(\ket{\psi}\) and a projection operator \(P\), the measurement projects \(\ket{\psi}\) onto the subspace corresponding to \(P\). The probability of the quantum state collapsing to the subspace defined by \(P\) is given by \(p = \bra{\psi} P \ket{\psi}\). After the measurement, if the outcome is associated with \(P\), the state collapses to \(\frac{P \ket{\psi}}{\sqrt{\bra{\psi} P \ket{\psi}}}\). Unlike projective measurements onto a complete basis set, general projection measurements may involve subspaces that do not span the entire Hilbert space. These types of measurements are useful for extracting specific information about a quantum system, such as determining whether the system lies within a particular subspace or has a particular property. General projection measurements are a crucial tool in quantum mechanics for analyzing and manipulating quantum states.

\end{comment}

\begin{comment}

\noindent\textbf{\textit{Quantum Mechanics, Quantization, and Second Quantization.}}
Quantum mechanics studies the theories for describing the behavior of nature at and below the scale of atoms.
One of the major studies is to quantize a physical system, referring to describing particles as wave functions.
One example is to quantize a many particle system via a Hamiltonian, a.k.a., Hermitian matrix.
There are two major usages of a quantization process: defining a Hamiltonian to picture the potential movement of particles
and simulating the quantum system by its Hamiltonian picturing.
Here is an analogy of the procedure. Defining a Hamiltonian equates to drawing a picture, or an initial snapshot, of a quantum state, potentially showing the possible movement of particles;
while simulating a quantum system, a.k.a., Hamiltonian simulation, is to see the trace behaviors based on the information provided by the initial snapshot.

{
\begin{center}
$
E=\bra{\psi(0)}\hat{H}\ket{\psi(0)}
\qquad
\qquad
\ket{\psi(t)}=\eexp{\hat{H} t}\ket{\psi(0)}
$
\end{center}
}

Two of the major Hamiltonian ($H$) applications are to compute the ground energy state for the initial quantum state $\ket{\psi(0)}$, as the fist formula above,
and to show the time-propagated simulation with respect to time $t$, i.e., the Schrodinger equation, as the second formula above.
We will explain the constructs shortly below.

Second quantization, i.e., the occupation number representation, is a common quantization method that describes the quantum system behaviors by viewing possible particle movements as electrons occupying certain orbits in different particle sites. Each particle site can be viewed as an $n$ dimensional dual Hilbert space. A creation or annihilation application can be viewed as pushing electron in a certain orbit to a higher or lower orbit, respectively. \qsnd formalizes the two operations in \Cref{sec:overview}.


\noindent\textbf{\textit{Quantum Value States}.} A quantum value
state\footnote{Most literature mentioned Quantum value states as \emph{quantum states}. Here, we refer to them as quantum value states or quantum values to avoid confusion between program and quantum states.  } %
consists of one or more quantum bits (\emph{qubits}), which can be expressed as a two-dimensional vector $\begin{psmallmatrix} \alpha \\ \beta \end{psmallmatrix}$ where the \emph{amplitudes} $\alpha$ and $\beta$ are complex numbers and $|\alpha|^2 + |\beta|^2 = 1$.
%
We frequently write the qubit vector as $\alpha\ket{0} + \beta\ket{1}$ (the Dirac notation \cite{Dirac1939ANN}), where $\ket{0} = \begin{psmallmatrix} 1 \\ 0 \end{psmallmatrix}$ and $\ket{1} = \begin{psmallmatrix} 0 \\ 1 \end{psmallmatrix}$ are \emph{computational basis-kets}. When both $\alpha$ and $\beta$ are non-zero, we can think of the qubit being ``both 0 and 1 at once,'' a.k.a. in a \emph{superposition} \cite{mike-and-ike}, e.g., $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$ represents a superposition of $\ket{0}$ and $\ket{1}$.
Larger quantum values can be formed by composing smaller ones with the \emph{tensor product} ($\otimes$) from linear algebra, e.g., the two-qubit value $\ket{0} \otimes \ket{1}$ (also written as $\ket{01}$) corresponds to vector $[~0~1~0~0~]^T$.
% 
However, many multi-qubit values cannot be \emph{separated} and expressed as the tensor product of smaller values; such inseparable value states are called \emph{entangled}, e.g.\/ $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$, known as a \emph{Bell pair}, which can be rewritten to $\Msum_{d=0}^{1}{\frac{1}{\sqrt{2}}}{\ket{dd}}$, where $dd$ is a bit string consisting of two bits, each of which must be the same value (i.e., $d=0$ or $d=1$). Each term $\frac{1}{\sqrt{2}}\ket{dd}$ is named a \emph{basis-ket} \cite{mike-and-ike}, consisting an amplitude ($\frac{1}{\sqrt{2}}$) and a basis $\ket{dd}$.

\end{comment}

%
%It is computationally hard to determine if an arbitrary quantum value is
%separable, therefore we say a general quantum value is \emph{possibly
%  entangled}.

%   
% An $n$-qubit quantum value state is typically represented as a $2^n$ dimensional
% vector. Alternatively, the values can be represented in different forms. For
% example, an initialized qubit typically has a value $\ket{0}$ or $\ket{1}$,
% called a \textit{normal typed value} ($\tnort$) in \qafny. A collection of $n$
% qubits that are in superposition but not entangled, i.e.,
% $\frac{1}{\sqrt{2}}(\ket{0} + \alpha(r_0)\ket{1})\otimes ... \otimes
% \frac{1}{\sqrt{2}}(\ket{0} + \alpha(r_{n-1})\ket{1})$, can be encoded as
% $\shad{2^n}{n\sminus 1}{\alpha(r_j)}$, where $\alpha(r_j)=e^{2\pi i r_j}$ and
% $r_j \in \mathbb{R}$, which is called a \textit{Hadamard typed value} ($\thadt$)
% in \qafny.

%Value $\alpha(r_j)$ is the \emph{local phase} of the state, which is a unique quantum amplitude whose norm is $1$, i.e., $\slen{\alpha(r_j)}=1$. 
%In the state $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$, we can view the local phase $1$ as $e^{0}$, and $\frac{1}{\sqrt{2^n}}e^{0}$ is the amplitude for every basis-ket.
%This is not a standard form for all unentangled multi-qubit value states but rather a convenient way of representing a particular class of states common in many quantum algorithms, which can be utilized for proof automation.

% The most general representation for $n$-qubit values is as a linear combination of basis-kets \cite{mike-and-ike}, or in
% Dirac notation in \cite{Dirac1939ANN}, as $\sch{m}{z_j}{\ket{c_j}}$, where $z_j\in \mathbb{C}$ is an amplitude, $c_j$ is an $n$-length bitstring called a \emph{basis} (computational basis only), and $m < 2^n$. The above notation is the same as ${z_0}\ket{c_0}+...+{z_{m}}\ket{c_{m}}$; each $j$-th element ${z_j}\ket{c_j}$ represents a \emph{basis-ket} in the superposition value state. 
% This is called an \textit{entanglement typed value} ($\tcht$) in \qafny.
% For example, the bell pair can be represented as $\sch{1}{\frac{1}{\sqrt{2}}}{\ket{c_j}}$ with $c_0=00$ and $c_1=11$.
% Notice that the basis-kets' bases ($c_j$) are all distinct in a value state. 
% \qafny identifies these three different representations and uses a type system to transform quantum-state representations properly.

%%Notice that the amplitudes satisfy the relation $\sum_{0}^{m}\slen{z_j}^2 = 1$. However, in some intermediate program evaluation in QNP, we lose the restriction to be $\sum_{0}^{m}\slen{z_j}^2 \le 1$, because a state $\sch{m}{z_j}{c_j}$ can be split into two parts as $\sch{m}{z_j}{c_j}=\schii{m_1}{z_i}{c_i}+\schk{m_2}{z_k}{c_k}$, and we might only want to reason about a portion of the state $\schii{m_1}{z_i}{c_i}$ locally so that $\sum_{0}^{m_1}\slen{z_i}^2 < 1$. 
%
%%In QNP, each quantum state is associated with a \emph{session}, referring to a cluster of quantum array pieces possibly entangled. We can view a session as a virtual quantum array that manages quantum physical qubit array pieces living in different locations but is locally connected through entanglement. See \Cref{sec:quantum-state}.


\noindent\textbf{\textit{Quantum Computations.}}

From the perspective of quantum mechanics, quantum computation can be viewed as a quantum simulation procedure based on the Schrödinger equation, involving unitary operations and quantum states. In this context, a quantum unitary operation may be defined as an exponential of a Hamiltonian.

Typical quantum computing theory often omits the explicit Hamiltonian and focuses on the computational aspects, treating the evolution of a quantum state as a sequence of \emph{quantum operations}, each acting on a subset of qubits in the quantum state. In standard presentations, quantum computations are expressed as \emph{circuits}. In these circuits, each horizontal wire represents a qubit, and boxes on these wires indicate quantum operations, or \emph{gates}. 

For example, the circuit to create a Bell pair uses two qubits and applies two gates: the \emph{Hadamard} (\texttt{H}) gate and a \emph{controlled-not} (\texttt{CNOT}) gate. Applying a gate to a state evolves the state. This evolution is mathematically expressed by multiplying the state vector by the gate's corresponding matrix representation; single-qubit gates are 2-by-2 matrices, and two-qubit gates are 4-by-4 matrices. The matrix representation of a gate must be \emph{unitary}, ensuring that it preserves the norm of the quantum state's amplitudes.

An entire quantum circuit can be described by composing its constituent gates into a single unitary matrix. This matrix representation encapsulates the overall transformation applied to the initial quantum state.

In our approach, we provide a time-dependent quantum mechanics perspective on quantum computation by incorporating both the Hamiltonian and time-propagation based on the time-dependent Schrodinger equation.




\begin{comment}

\noindent\textbf{\textit{Quantum Computations.}}
In the quantum mechanics point of view, quantum computation is a quantum simulation procedure based on the Schrodinger equation, including a unitary operation and a quantum state,
where a quantum unitary operation is defined as the exponential of a Hamiltonian.
A typical quantum computing theory omits the Hamiltonian layer and focuses on the simulation aspect, and view the computation on a quantum state consists of a series of \emph{quantum operations}, each of which acts on a subset of qubits in the quantum state. In the standard presentation, quantum computations are expressed as \emph{circuits}. In these circuits, each horizontal wire represents a qubit and boxes on these wires indicate quantum operations, or \emph{gates}. The circuit of a Bell pair uses two qubits and applies two gates: the \emph{Hadamard} (\coqe{H}) gate and a \emph{controlled-not} (\coqe{CNOT}) gate.
Applying a gate to a state \emph{evolves} the state. The semantics of doing so is expressed by multiplying the state vector by the gate's corresponding matrix representation; single-qubit gates are 2-by-2 matrices, and two-qubit gates are 4-by-4 matrices. A gate's matrix must be \emph{unitary}, ensuring that it preserves the unitarity invariant of quantum states' amplitudes. An entire circuit can be expressed as a matrix by composing its constituent gates.
In \qsnd, we provides the quantum mechanics view of quantum computation by including the Hamiltonian and simulation aspects.


\noindent\textbf{\textit{Quantum Measurement.}} 
%
A \emph{measurement} operation extracts classical information from a quantum value. It collapses the value to a basis state with a probability related to the value's amplitudes (\emph{measurement probability}), e.g., measuring $\frac{1}{\sqrt{2}}(\ket{0} + \ket{1})$ collapses the value to $\ket{0}$ with probability $\frac{1}{2}$,  and likewise for $\ket{1}$, returning classical value $0$ or $1$, respectively. 
A more general form of quantum measurement is \emph{partial measurement}, which measures a subset of qubits in a qubit array;
% 
such operations often have simultaneity effects due to entanglement, \ie{} in a Bell pair $\frac{1}{\sqrt{2}}(\ket{00} + \ket{11})$,
measuring one qubit guarantees the same outcome for the other --- if the first
bit is measured as $0$, the second bit is too.

In quantum mechanics, a projective measurement operator can be defined as a row vector, stated as a bra notation in the Dirac notation as $\bra{\psi}$.
For a quantum state $\ket{\psi}=\sch{m}{z_j}{\ket{d_j}}$, its row vector is $\bra{\psi}=\sch{m}{\sdag{z_j}}{\bra{d_j}}$.
Essentially, a row vector can be viewed as an adjugate transpose of a quantum state, i.e., $\bra{\psi}=\sdag{\ket{\psi}}$.
A projective measurement $\bra{\psi}$ on a quantum state $\ket{\psi}$ can be defined as $\braketa{\psi}{\psi}$,
resulting in a dot product of the row vector $\bra{\psi}$ and the state $\ket{\psi}$.
A projective measurement can also be viewed as a sequence of quantum gate applications followed by a computational basis measurement,
i.e., assume that we have a quantum unitary operation $e$, such that $e\ket{0}=\ket{\psi}$, then $\bra{\psi}=\sdag{\ket{\psi}}=\sdag{(e\ket{0})}$.
To avoid confusion, in the paper, we write a quantum state $\psi=\sch{m}{z_j}{\ket{d_j}}$ as a letter $\psi$, without the ket notation, and represent its row vector notation as $\sdag{\psi}$.
we overload our transpose operation, and define the transpose of a quantum state $\sdag{\psi}$ to be a row vector quantum measurement operation.

\end{comment}


\noindent\textbf{\textit{No Cloning and Observer Effect.}} 
The \emph{no-cloning theorem} suggests no general way of copying a
quantum value. In quantum circuits, this is related to ensuring the reversible
property of unitary gate applications.
% 
For example, the Boolean guard and body of a quantum conditional cannot refer to
the same qubits, e.g., $\qif{x[1]}{\qass{x[1]}{x[1]\, \splus\, 1}}$ violates the property as
$x[1]$ is mentioned in the guard and body.
% 
The quantum \emph{observer effect} refers to leaking information from a quantum value state. If a quantum conditional body contains a measurement or classical variable updates, it causes the quantum system to break down due to the observer effect. 
% 
\qafny{} enforces no cloning and no observer breakdown through the syntax and flow-sensitive type system.
}




==> case.tex <==
%\vspace{-0.3em}
\section{Extending QBlue to support Energy Computation}\label{sec:cases}

As we mentioned in \Cref{sec:overview2}, the third layer of semantics for a second quantization Hamiltonian is the application semantics to compute a ground energy state.
There are several algorithms that perform the task. One of the algorithms that naturally extends from Hamiltonian simulation is adiabatic quantum computation (AQC).
%
This is a model of quantum computation that solves optimization problems by evolving a quantum system slowly from a motion Hamiltonian $\hat{H}_m$ with a known ground state to a problem Hamiltonian $\hat{H}_p$ whose ground state encodes the solution. By maintaining the system's lowest energy state throughout the process, AQC leverages the adiabatic theorem to find optimal solutions efficiently. The first line below shows the time-dependent Hamiltonian $\hat{H}(r)$ that varies with time $r$ from $\hat{H}_m$ to $\hat{H}_p$. The Schr\"odinger equation on the right would give the exact evolution of this Hamiltonian. The actual solution used in AQC is the sequence on the second line, where each step generates a quantum operation via a Hamiltonian simulation ($\eexp{\uapp{\Delta r}{\hat{H}(r)}}$) for a small time period $\Delta r$. 
In theory, the AQC procedure can be understood as starting with an initial quantum state $\ket{\varphi(0)}$ and applying a sequence of unitary quantum operations, each of which is of the form $\eexp{\uapp{{\Delta r}}{\hat{H}(r)}}$ for a different $t\in\{\Delta r, 2\Delta r, 3 \Delta r, ...,T\}$. 

{\small
\begin{center}
$
\begin{array}{l}
\hat{H}(r)=(1-\frac{r}{T})\hat{H}_m + \frac{r}{T}\hat{H}_p
\qquad
\qquad
i\frac{d}{dt}\ket{\varphi(r)}=\hat{H}(r)\ket{\varphi(r)}
\\[0.4em]
\ket{\varphi(T)}\approx \eexp{\uapp{\Delta r}{\hat{H}(T)}} \circ ...\circ \eexp{\uapp{\Delta r}{\hat{H}(2\Delta r)}}\circ\eexp{\uapp{\Delta r}{\hat{H}(\Delta r)}}\ket{\varphi(0)}
\end{array}
$
\end{center}
}

We conceptually define a time-dependent Hamiltonian $\hat{H}(r)$ that evolves from $\hat{H}(0) = \hat{H}_m$ to $\hat{H}(1) = \hat{H}_p$ as a function of a normalized time parameter $r \in [0,1]$. For example, a linear schedule would use $\hat{H}(r) = (1-r) \hat{H}_m + r \hat{H}_p$. Initially ($r=0$) the system is in the ground state (eigenstate) of $\hat{H}_m$ (the initial superposition state). As $r$ increases, the Hamiltonian gradually incorporates the problem constraints. If the change is slow enough, the quantum adiabatic theorem guarantees that the state of the system will remain in the instantaneous ground state of $\hat{H}(r)$. By the end ($r=1$), the system will be in the ground state of $\hat{H}_p$, which is exactly the state encoding the optimal solution of our problem.
 
In practice, this continuous adiabatic evolution is realized through a sequence of many small discrete steps. Each step applies a slight alteration to the Hamiltonian and consequently a quantum operation on the state. Eventually, after the full schedule, the system's state ideally encodes the solution in its qubit amplitudes. Finally, we measure the qubits in the computational basis. With high probability (if the adiabatic process succeeded and if decoherence and other errors are minimal), the measurement will collapse the system into the basis state corresponding to the lowest energy, i.e., the optimal solution.

Adiabatic evolution replaces the explicit search or brute-force classical process with a physical process. As the Hamiltonian changes, the quantum state naturally ``searches'' the landscape of possibilities by continuously adjusting the amplitudes of basis-ket states, concentrating more weight on low-energy (better) solutions. By the end, the amplitude is ideally concentrated on the optimal solution. This is analogous to a landscape where the system begins as a liquid spread out over all valleys and then slowly freezes into the lowest valley (the global minimum) due to the energy bias introduced by $\hat{H}_p$. The power of this approach is that it exploits quantum parallelism and tunneling: the state can explore many solutions concurrently and avoid getting stuck in local minima under the right conditions, potentially outperforming certain classical algorithms on hard problems.


%\liyi{This section describes that we can extend the Hamiltonian simulation of QBlue language to other kinds, such as energy computation (via measurement vs VQE), and adiabatic computation. OR we can do case studies. }

%In this section, we show two case studies for the utility of \qsnd.

%\vspace{-0.3em}
%\subsection{The Quantum Interpretation of Clique Finding}\label{sec:clique} 

Here, we examine the use of the \qsnd dynamic semantics to perform AQC via a simple example in the $t(2)$ qubit system, and the full development of \qsnd AQC framework is one of our future works.
We present a quantum algorithm to find the largest clique in a random graph based on AQC \cite{farhi2000quantum}.
Given a graph $G=(V, E)$, we find if $G$ has a $k$-clique.
We assume a special initial superposition state $\psi(0)$, as a $ k$-Hamming weight superposition state, discussed shortly below.

{
\begin{center}
$
\hat{H}(r) = (1-\frac{r}{T})\hat{H}_m + \frac{r}{T}\hat{H}_p
\qquad
\underbrace{\eexp{r\hat{H}(n*r)}\circ...\circ\eexp{r\hat{H}(r)} \circ \eexp{r \hat{H}(0)}}_{n}
$
\end{center}
}

The whole algorithm can be understood as a loop structure, looping over $n$ steps of Hamiltonian simulation on $\hat{H}(r)$. We need to select a large enough time period $T$ so that the proper eigenstate $\psi(T)$, representing the largest clique, can be obtained.
We split the time period into small segments. For each segment $r$, we simulate $\eexp{{\uapp{r}{\hat{H}(j*r)}}}$ for $j\in[0,n]$, as the left equation above.
If the time segments are selected evenly, the number of Hamiltonian simulation iterations is $n=\frac{T}{r}$.

{\footnotesize
\begin{center}
$
\hat{H}_m = -\sum_{j,k} \sapp{\sdag{a}(j)}{a(k)}+\sapp{a(j)}{\sdag{a}(k)}
\quad
\hat{H}_p = -\sum_{j\neq m} (1\sminus E(j,m))\sapp{\mathbb{1}(j)}{\mathbb{1}(m)}
\quad
\psi_0 = 
\begin{pmatrix} n \\ k \end{pmatrix}^{-\frac{1}{2}}\sum\ket{z_k}^{\otimes n}
$
\end{center}
}


Here, $\hat{H}_m$ is the motion Hamiltonian, where the $k$-th Hamming weight superposition state is the eigenstate of the Hamiltonian, shown as the right above.
Every basis-vector in a $k$-th Hamming weight superposition state has exactly $k$ qubits marked as $\ket{1}$.
This state represents the collection of all $k$-subgraphs, i.e., the motion Hamiltonian represents that we quantumly search all $k$-th subgraphs.
The problem Hamiltonian $\hat{H}_p$ suggests that we observe every two different vertices $j$ and $m$ in a $k$-subgraph, by using the constraint $\sapp{\mathbb{1}(j)}{\mathbb{1}(m)}$ to indicate that the $j$-th and $m$-th vertices are included in the subgraph. In this case, we ensure an edge between the two vertices; otherwise, we add a penalty $(1\sminus E(j,m))$.

The initial state $\psi(0)$ is a superposition state of all the $k$-subgraph vertex sets ($k \le n$), similar to the one below, where $m_k=1$ if the vertex $k$ is in the subgraph.
If we model a basis vector $\ket{m_0}\ket{m_1}...\ket{m_{n\sminus 1}}$; each $m_k$ represents a vertex in the graph.

{\small
\begin{center}
$\begin{pmatrix} n \\ k \end{pmatrix}^{-\frac{1}{2}}
(
\ket{\underbrace{0...0}_{n}}
+
\ket{1\underbrace{0...0}_{n\sminus 1}}
+
\ket{01\underbrace{0...0}_{n\sminus 2}}
+
...
+
\ket{11\underbrace{0...0}_{n\sminus 2}}
+
...
+
\ket{\underbrace{11....1}_{n}}
)
$
\end{center}
}
%\vspace{-0.5em}

There are $\begin{pmatrix} n \\ k \end{pmatrix}$ different combinations of such vertex sets to form subgraphs.
The state preparation of such a superposition state can be another Hamiltonian simulation process mentioned in the work of \citet{10.5555/2011430.2011431}.
%
Through simulating (evolving) the Hamiltonian long enough, the system reaches its lowest energy state, the eigenstate $\psi(T)$. Upon measurement, it results in a candidate maximal clique in the graph, if there is any.
Unfortunately, it is impossible to foreknow the value to be used for $T$ for adiabatic evolution.
A solution is to include a classical post-measurement process that tries different values for $T$.
We can start by an initial guess of $T$, and if the AQC measurment result is not ideal, we can re-start the AQC process by increasing $T$ progressively to see if the system converges to a valid ground state.

%\vspace{-0.3em}
\ignore{
\subsection{Compiling Boson Particle Systems to Quantum Computers}\label{sec:boson} 

We show the compilation of a bosonic particle system for quantum computers.
Bosons are a special particle and typically require an infinite-dimensional Hilbert space to describe one spin, e.g., a one-spin boson is typed $t(1,\infty)$.
A typical way of approximating a bosonic system \cite{qua.25176} utilizes $2^{n\splus 1}$ dimensional Hilbert space, i.e., they use a length $n$ basis vector to track the particle state, representing a possible spot (orbital) for a particle to occupy, e.g., $\sdag{a}\ket{j}=\ket{j\splus 1}$ means that we zero the $j$-th position and mark the $j\splus 1$-th bit to be $1$.
The extra $n$-th position acts as an overflow bit, indicating if a maximal orbital is reached.
Essentially, the transformation from an $m$-particle bosonic system to a qubit system --- the Jordan-Wigner transformation for bosons \cite{qua.25176}) --- is a function $\gg^m:\quan{F}{\zeta}{\Motimes^m t(1,2^{n\splus 1})} \to \quan{F}{\zeta}{\Motimes^{m*(n\splus 1)} t(1,2)}$, compiling a $t(1,2^{n\splus 1})$ typed system to a $t(1,2)$ typed one, where the $t(1,2)$ typed system is written in the form of Pauli groups.
Since the bosonic system transformation is compositional, it is enough to show the transformation for one particle case $\gg:\quan{F}{\zeta}{t(1,2^{n\splus 1})} \to \quan{F}{\zeta}{t(1,2)}$, and view the $m$-particle case ($\gg^m$) as a map function by mapping $\gg$ to each particle in the system.
Apparently, the number of particles in the $t(1,2^{n\splus 1})$ and $t(1,2)$ typed systems ($m$ vs. $m*(n\splus 1)$) are different; thus, the particle site positions need to be rearranged.
In compiling a $t(1,2^{n\splus 1})$ system, we assume that a $j$-th position operation $op(j)$ is transformed to operations indexed $(j,0) ... (j,n)$, as $op'_0(j,0) ... op'_n(j,n)$, where the actual implementation of the $2D$ indices can be easily handled by a higher order function in $\lambda$-calculus.
To describe the transformation function $\gg$, it is enough to show the transformation of a $\quan{F}{\pmx}{t(1,2^{n\splus 1})}$ typed creators and annihilators below.

{\small
\begin{center}
$
\begin{array}{l@{\;\;}c@{\;\;}l@{\;}c@{\;}l}
 \sdag{a}(k):\quan{F}{\pmx}{t(1,2^{n\splus 1})} &\gg& \sum_{j=0}^{n\sminus 1}\sqrt{j\splus 1}(\sdag{a}\textcolor{spec}{(k,j)}:\quan{F}{\pmx}{t(1,2)} &\otimes& {a}\textcolor{spec}{(k,j\splus 1)}:\quan{F}{\pmx}{t(1,2)})
\\[0.4em]
a(k):\quan{F}{\pmx}{t(1,2^{n\splus 1})} &\gg& \sum_{j=0}^{n\sminus 1}\sqrt{j\splus 1}(a\textcolor{spec}{(k,j)}:\quan{F}{\pmx}{t(1,2)} &\otimes& \sdag{a}\textcolor{spec}{(k,j\splus 1)}:\quan{F}{\pmx}{t(1,2)})
\end{array}
$
\end{center}
}

The indices in \textcolor{spec}{blue} in the right-hand expanded tensor form only serve indicator purposes.
The compilation of $t(1,2)$ typed creators and annihilators to Pauli operations is a direct result of \Cref{eq:pauli}, shown below.

{\small
\begin{center}
$
\sdag{a}:\quan{F}{\pmx}{t(1,2)}= \frac{1}{2}(X + i Y)
\qquad
a:\quan{F}{\pmx}{t(1,2)}= \frac{1}{2}(X - i Y)
$
\end{center}
}

We now see an application of transforming a two-particle bosonic system, with $n=1$, to quantum computers for simulating the boson behavior based on the Bose-Hubbard system \cite{peng2023quantum}, an instantiation of the Hubbard system (as an abstract class) \Cref{eq:hubbard} to describe the superconducting behaviors of boson particles.
Similar to the Hubbard system, a two-particle Bose-Hubbard system comprises of an expression $\sapp{\sdag{a}(0)}{a(1)}+\sapp{a(0)}{\sdag{a}(1)}$, referring to that index $0$-th and $1$-st particles might be exchanged in the next moment. The system also contains the repulsion term, similar to the one in \Cref{eq:hubbard}.

We now see how to compile a subterm of the two-particle system, $\sapp{\sdag{a}(0)}{a(1)}+\sapp{a(0)}{\sdag{a}(1)}$, to quantum computers.
Such an expression is syntactic sugar, similar to the $\lambda$-calculus term in \Cref{sec:sim-gates}.
A simplified version of the expanded expression is ${\sdag{a}\textcolor{spec}{(0)}}\otimes {a\textcolor{spec}{(1)}}+{a\textcolor{spec}{(0)}}\otimes {\sdag{a}\textcolor{spec}{(1)}}$, obtained by expanding the tensor products to show the position relations among different operations.
Note that we omit the type annotations $\quan{F}{\pmx}{t(1,2^{2})}$ in the term for simplicity.
By using the above transformation function, we can transform the system to a $t(1,2)$ typed one, named $\hat{H}_T$, as:

{\footnotesize
\begin{center}
$
\begin{array}{c@{\;\;}l}
&
\;
(\sdag{a}\textcolor{spec}{(0,0)}:\quan{F}{\pmx}{t(1,2)} \otimes {a}\textcolor{spec}{(0,1)}:\quan{F}{\pmx}{t(1,2)})\otimes (a\textcolor{spec}{(1,0)}:\quan{F}{\pmx}{t(1,2)} \otimes \sdag{a}\textcolor{spec}{(1,1)}:\quan{F}{\pmx}{t(1,2)})
\\[0.2em]
&
\quad
+(a\textcolor{spec}{(0,0)}:\quan{F}{\pmx}{t(1,2)} \otimes \sdag{a}\textcolor{spec}{(0,1)}:\quan{F}{\pmx}{t(1,2)})
\otimes
(\sdag{a}\textcolor{spec}{(1,0)}:\quan{F}{\pmx}{t(1,2)} \otimes {a}\textcolor{spec}{(1,1)}:\quan{F}{\pmx}{t(1,2)})
\\[0.3em]
=&
\frac{1}{2}(X + i Y) \otimes \frac{1}{2}(X - i Y) \otimes \frac{1}{2}(X - i Y) \otimes \frac{1}{2}(X + i Y)
+
\frac{1}{2}(X - i Y) \otimes \frac{1}{2}(X + i Y) \otimes \frac{1}{2}(X + i Y) \otimes \frac{1}{2}(X - i Y)
\\[0.3em]
=&
\frac{1}{8}(X\otimes X \otimes X \otimes X + X\otimes X \otimes Y \otimes Y+Y\otimes Y \otimes X \otimes X + Y\otimes Y \otimes Y \otimes Y
\\[0.1em]
&\quad\qquad+ X\otimes Y \otimes X \otimes Y + X\otimes Y \otimes Y \otimes X + Y\otimes X \otimes X \otimes Y + Y\otimes X \otimes Y \otimes X)
\end{array}
$
\end{center}
}

}






==> overview.tex <==
\subsection{QBlue: Second Quantization Language as Energy Constraint Programming}\label{sec:overview2}

The \qsnd language is based on second quantization. We first examine QBlue's programmability for directing users to write energy constraint programs, mainly to answer the question how scientific computation users think of Hamiltonian programs.
Recall that the Hamiltonian constraint for $K$-clique finding is  $\sum_{j\neq m} (1.0-E(j,m)) * \sapp{\mathbb{1}(j)}{\mathbb{1}(m)}$, where we search all the $k$-subgraphs and add penalties for pairs of vertices $j$ and $m$ in a subgraph that has no edge. If we compute the Hamiltonian energy value for a subgroup to be $0$, the subgroup is a clique. Such constraint programming can be done in adiabatic quantum computing.

Quantum particle system Hamiltonian essentially adopt this kinds of Hamiltonian constraint concepts.
We first show a Hubbard Model example \footnote{Simplified version, and a full version is in \Cref{sec:hubbard}.}, used to describe the tunnelling of quantum particles in one site to the other by viewing sites are managed as a lattice graph.
%The lattice graph and site concept is essentially a generalization of the quantum circuit diagram in \Cref{sec:background3},
%in the sense that each qubit is a site, operations in each circuit line represents a sequence of operation applying to the site, and multi-qubit opertions represent interactions across different sites. Defining Hamiltonian constraints based on the generalized lattice graph and site concept provides additional freedom for users to restrict how sites can communicate, e.g., we can restrict that some circuit lines in \Cref{sec:background3} are not capable of communication.
The Hamiltonian below operates on sites holding fermions, described by two dimensional Hilbert space ($\Hilb_2$).

{\small
\[
\hat{H} = \sminus z_t \sum_{j} 
\left(\sapp{\sdag{a}(j)}{ a(j\splus 1)} + \sapp{\sdag{a}(j\splus 1)}{ a(j)}\right) + z_u \sum_{j}  \sapp{\mathbb{1}(j)}{\mathbb{1}(j\splus 1)}
\tag{2.3.1}\label{eq:hubbard}
\]
}

Before we examine the program behavior, we first identify three layers of Hamiltonian program semantics for any Hamiltonian systems below.

\begin{itemize}
\item \emph{Constraint Semantics} refers to that a Hamiltonian represents a Hermitian matrix, applicable to a state; such semantics describes the constraint among different particle sites and the operations represent quantum constraints user's intention for a system.
\item \emph{Dynamic Semantics} refers to Hamiltonian simulation ($\eexp{{\hat{H}}{t}}$), where we learn about the state at time $t$, as $\psi(t)$, by simulating the Hamiltonian $\hat{H}$ on the initial state $\psi(0)$, as $\eexp{{\hat{H}}{t}}\psi(0)$; such simulation produces a unitary implementable in quantum computers.
\item \emph{Ground Energy Semantics} refers to finding the a \emph{minimized energy state} $\psi_{min}$ minimizing the constraints defined in $\hat{H}$, defined as $\cn{min}(\hat{H})$.
\end{itemize}

This paper does not formalize ground energy semantics, as we show an example computation via adiabatic quantum computation method in \Cref{sec:cases}.
%The second layer is the Hamiltonian dynamic semantics in this paper, defined by the Hamiltonian simulation ($\eexp{\sapp{\hat{H}}{t}}$), referring to that we learn about the state at time $t$, as $\psi(t)$, by simulating the Hamiltonian $\hat{H}$ on the initial state $\psi(0)$.
%The third layer is the application semantics, defined by $\cn{min}(\hat{H})$, computing out a \emph{minimized energy state} $\psi_{min}$ minimizing the constraints defined in $\hat{H}$.
%We show a way of computing the minimized energy state via adiabatic quantum computation method in \Cref{sec:cases}.

We examine the constraint level program behavior of Hamiltonian programs. The Hubbard model program is similar to many other Hamiltonian constraint programs \cite{10.3389/fphy.2014.00005,10.21468/SciPostPhys.8.2.021}, where the program can be partitioned into an initial Hamiltonian and a final Hamiltonian, connected by a sum operation. In this paper, we classify initial Hamiltonians as motion Hamiltonians $\hat{H}_{m}$ and final Hamiltonians as problem Hamiltonians $\hat{H}_p$, where the names indicate the constraint behavior.

If we view the ket numbers in each site as the number of particles occupying in the site,
motion Hamiltonians define the constraints for the potential particle movement in different sites.
The motion Hamiltonian $\sminus z_t \sum_{j} (\sapp{\sdag{a}(j)}{ a(j\splus 1)} + \sapp{\sdag{a}(j\splus 1)}{ a(j)})$ indicates that the appearance of a particle in the $j$-th site ($\sdag{a}(j)$) results in the particle disappearance in the $j\splus 1$-th site, and vice versa.


\begin{wrapfigure}{r}{3.3cm}
%\vspace*{-2.5em}
  \includegraphics[width=0.25\textwidth]{demo.pdf}
%\vspace*{-0.5em}
  \caption{Analogy}
%\vspace*{-1em}
\label{fig:analogy}
\end{wrapfigure}

Another common motion Hamiltonian is $\sum_{\cn{j}=0}^n(\sdag{a}(j)+a(j))$, e.g., applying Pauli $X$ to every $j$-th site. 
An $n$ qubit uniform superposition state $\frac{1}{\sqrt{2}}\sum_{k=0}^{2^n} \ket{k}$ is the eigenstate of the motion Hamiltonian.
To understand the program behavior of the motion Hamiltonian,
its Hamiltonian simulation is as if there is an assembly line, and each worker is dealing with a single basis-ket in the superposition state.
As demonstrated in the analogy in \Cref{fig:analogy}, Alice and Bob are two workers dealing with two basis-kets.
Applying an operation $\sdag{a}(j)+a(j)$ on the first qubit means that we make a product shift of the assembly line based on the first position of each basis-ket so that Alice and Bob swap the basis-kets they were dealing.

Problem Hamiltonians, e.g., the $\hat{H}_p = z_u \sum_{j}  \mathbb{1}(j) \circ \mathbb{1}(j\splus 1)$ in the Hubbard model, represent the particle properties in a problem. $\hat{H}_p$ can be rewritten as  $z_u \sum_{j} (\mapp{\sdag{a}(j)}{a(j)}) \circ (\mapp{\sdag{a}(j\splus 1)}{ a(j\splus 1)})$.
Recall that $\mathbb{1}$ stabilizes $\ket{1}$ state. The $\hat{H}_p$ constraint semantics suggests that if two adjacent sites showing both $\ket{1}$, we apply a penalty ($z_u$) constraint to the system and the simulation of the system should reach a state minimizing energy penalties.
%Particularly, the problem Hamiltonian in the Hubbard model suggests that we want to add a penalty $z_u$, if two adjacent sites having occupied particles ($\ket{1}$).
%In the above Hubbard model program, the term $\mapp{\sdag{a}(j)}{ \mapp{a(j)}{\mapp{\sdag{a}(j\splus 1)}{ a(j\splus 1)}}}$ means we applying two $\mathbb{1}$ ($\mapp{\sdag{a}}{a}$) operations to two adjacent sites ($j$ and $j\splus 1$), referring to that we impose a penalty constraint if two adjacent sites are occupied by two fermions.

\subsection{The QBlue Compiler and Optimization Algorithms}\label{sec:sim-gates}

%\liyi{This section overviews the compiler with figures, and an example.}
Hamiltonians represent constraints that users intend to do, which are not directly compilable.
Typically, we compile Hamiltonian simulation \cite{Tacchino_2019,Li_2022,cao2024marqsimreconcilingdeterminismrandomness,10.1145/3503222.3507715}, the dynamic semantics, to quantum computers for execution. We dicuss below the key \qsnd features to compile Hamiltonian simulation.

\noindent{\textbf{\emph{Adding Types in \qsnd.}}}
%
Without specifying the two-dimensional fermion state indication, one cannot determine what kind of systems that the Hubbard model Hamiltonian constraint describes, e.g., the same program can be used to describe a boson system \cite{peng2023quantum}.
To constrain the system for fermions, \qsnd types each site as $t^{\aleph}(2)$, referring to a two-dimensional fermion state.
\qsnd also classifies a qubit system above having $t(2)$ typed sites, as a qubit and a $t(2)$ typed boson behave the same.
The types can help classify different sites in \qsnd and permit the interactions of different quantum particles.
We permit other particle types; see \Cref{sec:formal}.
The typing is useful when transforming a particle system to another, often in analyzing different particle systems.
For example, when compiling a two particle $t(m)$ typed system $\hat{H}$, with typing $t(m) \otimes t(m)$, to a qubit system with each site being $t(2)$ type,
we notice that a basis-vector state $j \in [0,m)$ in a particle, whose binary form can be represented by a bitstring with the length $N=\ulcorner \log(m) \urcorner$.
The above two particle system can be compiled to a $\Motimes^{2*N}$ typed qubit system, each qubit is typed as $t(2)$. If we consider the two particle system Hamiltonian simulation as a function $\Motimes^2 t(m) \to \Motimes^2 t(m)$, the compilation is a high-order function below.

{
\begin{center}
$
(\Motimes^2 t(m) \to \Motimes^2 t(m)) \to (\Motimes^{2*N} t(2) \to \Motimes^{2*N} t(2))
$
\end{center}
}

%Our type construct, $t(n,m)$, also crystallizes the spin concept in our second quantization formalism.
%Recall in \Cref{fig:data} that the $t(n,m)$ type essentially represents tensors of Hilbert space ${\bigotimes^{n}{\mathpzc{H}^{m}}}$ for describing each particle site, and each Hilbert space describes a spin.
%One can think of the spins as if we have $n$ different counters in a particle site, and applying an operation with a spin flag refers to applying it to the right counter.
%To understand the concept clearly, let's focus on the $t(2,2)$ typed particle case, which has two possible spins.
%Here, \(\ket{1}_0\ket{0}_1\) (written as \(\ket{\uparrow}\) in some literature) means that a particle site contains a spin-up ($\uparrow$) electron, while \(\ket{0}_0\ket{1}_1\) (traditionally written as \(\ket{\downarrow}\)) refers to a particle site containing a spin-down ($\downarrow$) electron. Obviously, applying a annihilator $a_{0}$ to \(\ket{1}_0\ket{0}_1\) results in \(\ket{0}_0\ket{0}_1\) (traditionally written as \(\ket{0}\)) and applying a creator $a_{1}$ to the above state results in \(\ket{1}_0\ket{1}_1\) (traditionally written as \(\ket{\uparrow\downarrow}\)).
%The \qsnd type information clarifies the spin behaviors, as some systems \cite{10.1145/3632923} misinterpreted spin-up and down as qubits $\ket{0}$ and $\ket{1}$ without proper compilation.
%As we show here, they are not identical.

\noindent{\textbf{\emph{A Complete and End-to-End Compilation.}}}
Previous Hamiltonian simulation compilation works are either example-based \cite{Li_2022,Tacchino_2019} without formalism, or focus on specific subroutines, such as Trotterizations \cite{cao2024marqsimreconcilingdeterminismrandomness,10.1145/3503222.3507715}.
\qsnd intends to provide the first end-to-end compilation formalism for compiling Hamiltonian simulation for any second quantization Hamiltonian programs to quantum circuits, both digital and analog based.
%Finding the right target machine Hamiltonian to simulate a gate, i.e., gate synthesis, is usually referred to as control pulse level quantum programming \cite{Li_2022,Tacchino_2019} as control pulses can theoretically be described as \emph{target machine Hamiltonians}, and previous work \cite{10.1145/3632923} has discovered the advantage of compiling system Hamiltonians directly to target machine Hamiltonians by bypassing the series of simulations of individual gates.
To see how our compiler works, we simulate a simple $t(2)$ typed Ising model system $\hat{H}_{I1}$ on the left below, describing phase transition and quantum magnetism behaviors in insulating magnetic systems.

{\small
\[
z_h \sum_j \big(\sdag{a}(j) + a(j) \big) + \sum_{j} {\big(\mathbb{0}(j) - \mathbb{1}(j)\big)}\circ {\big(\mathbb{0}(j\splus 1)-\mathbb{1}(j\splus 1)\big)}
\looongrightarrow
 z_h \sum_j X(j) + \sum_{j} {Z(j)}\circ{Z(j\splus 1)}
 \tag{2.4.1}\label{eq:ising}
\]
}


\begin{figure*}[t]
{\small
\begin{tabular}{c@{$\;\;=\;\;$}c}
\begin{minipage}{0.22\textwidth}
$
\eexp{\frac{r}{n}{\sapp{Z(j)}{Z(j\splus 1)}}}
$
\end{minipage}
&
\begin{minipage}{0.3\textwidth}
{
  \Qcircuit @C=0.5em @R=0.5em {
    \lstick{} & & \ctrl{1}       & \qw  & \ctrl{1}      &\qw\\
    \lstick{} & & \targ         & \gate{\cn{Rz}(2\frac{r}{n})}       & \targ    & \qw 
    }
}   
\end{minipage}
\end{tabular}
\hspace{1em}
\begin{minipage}{0.41\textwidth}
{\small
$
ZZ(\theta)=
\begin{psmallmatrix}
\cn{exp}(\sminus i\frac{\theta}{2}) & 0 & 0 & 0\\
 0 & \cn{exp}(i\frac{\theta}{2}) & 0 & 0\\
 0 & 0 & \cn{exp}(i\frac{\theta}{2}) & 0\\
 0 & 0 & 0 & \cn{exp}(\sminus i\frac{\theta}{2})
\end{psmallmatrix}
$
}
  \end{minipage}
}
\vspace*{-0.8em}
\caption{Circuit and unitary for $ZZ$ Interaction. The left circuit applies on $j$ and $j\splus 1$ qubits.}
\label{fig:zz-inter}
\vspace*{-1.2em}
\end{figure*}

The term in $\hat{H}_{I1}$, $z_h \sum_j \sdag{a}(j) + a(j)$, is the motion Hamiltonian constraining potential movements, and the second sum term is the problem Hamiltonian constraining the energy penalties. If two adjacent sites have the same kets (both $\mathbb{0}$ or $\mathbb{1}$), there is a positive energy penalty, while if the two sites have opposite ket states (having one $\mathbb{0}$ and $\mathbb{1}$), there is a neative energy penalty representing an incentive. Thus, the problem Hamiltonian constrains that two adjacent sites describe magnet forces.

To compile the Hamiltonian simulation $\eexp{\hat{H}_{I1} r}$ with respect to a time $r$ (in \qsnd, we typically write $r$ as amplitudes of Pauli operators in $\hat{H}_{I1}$), we first perform particle transformation (\Cref{sec:transformation}) to transform the system to a Pauli-based Hamiltonian, a.k.a., a sum of Pauli strings, as the right above. The main step in compiling the Pauli-based Hamiltoinan simulation is Trotterization, a technique to split $\hat{H}_{I1}$ into small Hamiltonians, and perform Hamiltonian simulation for the smaller Hamiltonians in sequence to approxmate $\eexp{\hat{H}_{I1} r}$.
In the above example, Trotterization produces a sequence of $\eexp{\frac{r}{n} {Z(j)}\circ{Z(j\splus 1)}}$ and $\eexp{\frac{r}{n} X(j)}$ operations (the sequence length is related to $n$). If $n$ is large enough, the operation sequence is a good approximation to $\eexp{\hat{H}_{I1} r}$.
The $\eexp{\frac{r}{n} X(j)}$ operation produces a \cn{Rx} gate \cite{mike-and-ike}, while $\eexp{ \frac{r}{n} {Z(j)}\circ{Z(j\splus 1)}}$ produces a digital circuit as the left in \Cref{fig:zz-inter}, performing two controlled-not gates and an $\cn{Rz}(2\frac{r}{n})$ gate in the middle for the $j$-th and $j\splus 1$-th qubits,
i.e., $\cn{Rz}(\theta)$ is an $z$-axis phase rotation gate, rotating $\theta$ angle.

There are also analog-based compilation compiling Hamiltonian simulations to target machine Hamiltonians by viewing quantum computers as a Hamiltonian simulator.
For example, IBM provides a direct programming support for $ZZ$ interaction gate shown as the right in \Cref{fig:zz-inter}; the special gate essentially simulates the target machine Hamiltonian $\sapp{Z(j)}{Z(j\splus 1)}$ in a much more effective way than the above digital circuit gate synthesization step.

%As we mentioned above, these quantum gates are eventually simulated as Hamiltonians in pulse-level programming.

%On the other hand, instead of performing the sequence of the three gate simulations above,
%one can directly implement the small Hamiltonian in an IBM machine, which supports direct pulse level programming and provides the $ZZ$ interaction gate shown as the right in \Cref{fig:zz-inter}; the special gate essentially simulates the target machine Hamiltonian $\sapp{Z(j)}{Z(j\splus 1)}$ in a much more effective way than the above gate synthesis step.
%The bypassing shows the potential of improving the compilation effectiveness.
%In many cases, even if one is willing to implement system Hamiltonians as circuit gates, it is still valuable for them to notice the potential optimization done through the above procedure, definable in \qsnd, as many optimization frameworks \cite{VOQC,10.1145/3519939.3523433} decompose a $ZZ$ gate as the three gates above, which is counterproductive.





\begin{comment}

\ignore{


We first describe the state structure and operations for a single particle. The \qsnd single particle state structures and types are illustrated in \Cref{fig:data}. Each particle state represents a quantum state snapshot of the number of electrons occupying a particular site and can be expressed as a dual Hilbert space \(\hspb{n}\), also known as a pair of \(n\)-dimensional Hilbert spaces.

In \qsnd, each single particle state \(\sum_j \dualm{z_j}{k_j}{m_j}\) is a linear combination of basis-kets \(\dualm{z_j}{k_j}{m_j}\). Each basis-ket consists of a complex amplitude value \(z\), and two basis vectors \(\ket{k}_{\uparrow}\) and \(\ket{m}_{1}\) with natural numbers \(k\) and \(m\). Many literature works describe their systems using basis-ket symbols \(\ket{\uparrow}\), \(\ket{1}\), and \(\ket{0}\), which are represented as \(\dualm{}{1}{0}\), \(\dualm{}{0}{1}\), and \(\dualm{}{0}{0}\) in \qsnd. The basis-ket formalism extends from the Dirac notation \cite{Dirac1939ANN}, marking a ket, e.g., \(\ket{k}\), with spin flags (\(\uparrow\) and \(1\)). Each state is associated with a single particle type \(\hspb{n}\), and the basis vector numbers \(k\) and \(m\) are in the range \([0,n)\). For example, a basis vector in a two-dimensional dual Hilbert space can be \(\ket{0}\) or \(\ket{1}\).

The spin operator (\(\sigma\)) represents the spin state of a particle, potentially being in the up (\(\uparrow\)) or down (\(1\)) positions. For example, \(\dualm{}{1}{0}\) (sometimes written as \(\ket{\uparrow}\)) means that a particle site contains a spin-up electron, while \(\dualm{}{0}{1}\) (sometimes written as \(\ket{1}\)) refers to a particle site containing a spin-down electron. Sometimes, users may ignore the spin operators in their analyses. In such cases, particles are assumed to be always spin-up (\(\dualm{z}{k}{0}\)) and abbreviated as \(z\ket{k}\).

In \qsnd, we include a zero state value \(\zero\), which adheres to the identity equation property (\(\zero + v = v\)).

A single particle operation in second quantization represents the potential modification of electrons in a particle site (state snapshot), analogous to the increments or decrements of basis vector numbers in a basis-ket. Typically, a creation operation (\(a^{\dag}\)) increments the basis vector number, and an annihilator (\(a\)) decrements the basis vector number. Each single particle operation is also labeled with spin flags (\(a_{\uparrow}\) and \(a_{1}\)) to manipulate the spin-up and spin-down basis vectors of a basis-ket, respectively. The semantics of applying an annihilator to a single basis-ket are summarized in rules \rulelab{S-AUB}, \rulelab{S-AUN}, \rulelab{S-ADB}, and \rulelab{S-ADN} in \Cref{fig:sem}. An annihilator with a specific spin flag \(\sigma\) reduces the basis vector number in the ket with the same flag \(\sigma\), if the number is not zero; otherwise, the application results in a zero state (\(\zero\)).

These rules apply to single basis-kets (without amplitude values). In general, applying such an operation to a quantum state that might be in superposition (a linear combination of basis-kets) results in a linear combination of applying the operation to different single basis-kets. Conversely, a creator (\(\sdag{a}_{\sigma}\)) increments the basis vectors, as summarized below. Each creator application is associated with the \(n\) value from the type (\(\hspb{n}\)) of the state to which the creator is applied.

{\small
\begin{center}
$
\begin{array}{l@{\;\;}c@{\;\;}l@{\qquad}l@{\;\;}c@{\;\;}l}
\sdag{a}_{\uparrow}\dualm{}{k}{m} &\longrightarrow& \zero & \sdag{a}_{1}\dualm{}{k}{m} &\longrightarrow& \zero 
\\[0.8em]
\sdag{a}_{\uparrow}\dualm{}{k}{m} &\longrightarrow& \dualm{}{k\splus 1}{m} \;\; \cn{if}\; k \neq n &
\sdag{a}_{1}\dualm{}{k}{m} &\longrightarrow& \dualm{}{k}{m\splus 1} \;\; \cn{if}\; m \neq n
\end{array}
$
\end{center}
}

In \qsnd, the second quantization operations are modeled using only annihilators (\(a\)), and a creator is defined as the transpose (\(\sdag{e}\)) of an annihilator.

The above \qsnd data and operation definitions formalize the behavior of a single particle site. To connect different particles, we utilize a tensor operation \(\otimes\), i.e., \(v_1 \otimes v_2\) connects two single particle states, and \(e_1 \otimes e_2\) connects two operations. For example, the composition of two particle states can be expressed as \(v \otimes v'\), and we adopt the following abbreviation:

{\small
\begin{center}
$
\dualm{}{k_1}{m_1} \otimes \dualm{}{k_2}{m_2} = \dualm{}{k_1}{m_1} \dualm{}{k_2}{m_2}
\qquad
\sum_j z_j \eta_j \otimes \sum_k z_k \eta_k = \sum_{j,k} (z_j \cdot z_k) \eta_j \eta_k
$
\end{center}
}

To express entangled quantum states across different particles, we denote the \(n\)-particle state form as \(\sum_j z_j \eta_{1j} \eta_{2j} \ldots \eta_{nj}\), an extension of Dirac notation with spin flags. Essentially, a tensor product can be viewed as a location separation in a system. Applying a tensor product of operations to a state means applying each operation to the appropriate location in every basis-ket in the state. For example, \(a_{\uparrow} \otimes \sdag{a}_{1}\) means applying the first annihilator (\(a_{\uparrow}\)) to the first particle site and the creator (\(\sdag{a}_{1}\)) to the second particle. If the state is \(\sum_{j,k} (z_j \cdot z_k) \eta_j \eta_k\), the application will be:

{\small
\begin{center}
$
\sapp{(a_{\uparrow} \otimes \sdag{a}_{1})}{(\sum_{j,k} (z_j \cdot z_k) \eta_j \eta_k)} \longrightarrow \sum_{j,k} (z_j \cdot z_k) (\sapp{a_{\uparrow}}{ \eta_j}) (\sapp{\sdag{a}_{1}}{ \eta_k})
$
\end{center}
}

Additionally, we allow a linear sum operation \(e_1 + e_2\), performing a linear sum, i.e., applying \(e_1 + e_2\) to a state \(v\) means \((\sapp{e_1}{v}) + (\sapp{e_2}{v})\). A sum operation might produce superposition if \(v\) is a state just initialized as a tensor product of basis-kets, which can be thought of as a \emph{quantum choice} operation, in the sense that one can perform either \(e_1\) or \(e_2\) to the state \(v\) at the same time. We also permit a function sequencing operation \(\sapp{e_2}{e_1}\), consecutively applying \(e_1\) and \(e_2\) to a state. Essentially, the sequencing operator \(\sapp{e_2}{e_1}\) is an abbreviation of \(\lambda x . \sapp{e_2}{(\sapp{e_1}{x})}\), where \(x\) is a state. More information is in \Cref{sec:formal}.


\amr{The single particle state (Fig.3) makes sense. The tensor product is clearly motivated. The linear sum operation appears too low-level of a way to introduce superpositions. There should be restrictions on $e_1$ and $e_2$, right? Is the sum reversible?}

\liyi{The simulation, which produces a unitary, is reversible. To produce a unitary, you will need to define a Hamiltonian, and the exponent of the Hamiltonian is a unitary. A single creator/annihilator does not produce a Hamiltonian (Hamiltonian requires a Hermitian matrix, which can be checked in our type system). }

\liyi{The requirement of a sum is a quantum state that needs to be normalized. }

\amr{I have a major idea: if we remove the linear sum (and the $\Sigma$ values), do we essentially get a classical language ? Wouldn't the presentation be much more clear, if we presented the classical core first with examples, types, etc. In that classical core, we still have creation / annihilation, tensor products, unitary (permutation) matrices, and lambda terms. We can provide some simple examples. Then we add the linear sum operation, generalize values to $\Sigma$, and the entire thing turns quantum but it would be much easier to understand. }

\liyi{Yes, actually you are correct. }

\amr{On a related note, what is the role of the $\lambda$-calculus? One obvious role is to provide sequential composition and recursion. But is there any particular need for higher-order functions? } 

\liyi{The lambda-typed calculus provides a way of unifying operations and quantum states in the same system, so quantum states are now values in the system. In addition, it provides a way of clasifying sites. In our system, two different sites might not have the same state types, i.e., one might be an electron, and the other might be a nucleus. So The former can be described by a two dimensional and the later are described by high dimensional. }


In this section, we use an simple $1D$ and general transverse-field Ising systems as running examples below, which describes phase transition and quantum magnetism behaviors in insulating magnetic systems and order-disorder ferroelectrics.

{\small
\[
\hat{H}_{I1} = \sum_{j} \sapp{Z(j)}{Z(j\splus 1)} + z_h \sum_j X(j)
\qquad
\qquad
\hat{H}_{IG} = \sum_{j,m} \sapp{z_{J}}{\sapp{Z(j)}{Z(m)}} + z_h \sum_j X(j)
\]
}

The $\hat{H}_{I1}$ equation is a special $1D$ Ising system with uniformed interaction strength and it describes a $1D$ lattice structure,
while the $\hat{H}_{IG}$ equation is a general Ising system, where every two particles are connected regardless lattice structures.
In both equations, the first terms in the quantum choice represent the particle interactions, while the second terms represent effects from external transverse magnetic field.
$z_J$ is the interaction strength, describing the connection magnitudes between different particles, while $z_h$ is the external transverse magnetic field strength.

The reason that a quantum choice term can be turned into additional effects applying to a system is the same as the one in the Hubbard model system (\Cref{sec:hubbard}),
where the application of the additional term to a quantum state acts like an incentives, increasing or decreasing the probability amplitudes of certain basis-kets,
if we view basis-kets as states that particles can hold.
In physics, particle interactions are typically modeled as a sequencing operation, as $\sapp{Z(j)}{Z(j\splus 1)}$ and $\sapp{Z(j)}{Z(m)}$ above,
because this directly models the traces of particle movements.
Recall that Hamiltonians represents particle state snapshots.
In describing two particle interactions in a Hamiltonian, it is enough to put down formulas that describe how both of the two particles move towards in the snapshot.
Here, the sequencing operation describes the two particles, $j$ and $j\splus 1$ in the $1D$ case and $j$ and $m$ in the general case,
potentially rotating along the $z$-axis, with an additional forces from the $x$-axis because of the external transverse magnetic field. 

One key application to the simulation of a quantum system, i.e., given a state $v$ and a simulation time slot $t$, to simulate $\hat{H}_{I1}$ at time $t$,
we compute the matrix exponent $\eexp{\sapp{\hat{H}_{I1}}{t}}$ and apply on the state $v$; such application produces a quantum state $v'$ representing the state of simulating the system at time $t$.
Notice that the exponent of a Hamiltonian is a unitary matrix, implementable in a quantum computer.
Obviously, the produced unitary might be too complicated and require the compilation to circuit gates in quantum computers, which is done by Trotterization \cite{Lloyd96},
based on Lie-Trotter product formula \cite{Lie1880}, as the left term below.

{\small
\begin{center}
$\cn{exp}(A+B)=\lim_{n\to \infty}\left(\sapp{\cn{exp}({\frac{A}{n}})}{\cn{exp}({\frac{B}{n}})}\right)^n
\qquad
\qquad
\cn{exp}(\delta(A+B))=\sapp{\cn{exp}(\delta(A))}{\cn{exp}(\delta(B))}+O(\delta^2)
$
\end{center}
}

The right term above is the approximated formula developed by Suzuki \cite{529425},
which suggests that the error rate $O(\delta^2)$ is related to the square of the variable term $\delta$.
In the context of quantum simulation, $\delta$ refers to the $\sminus \sapp{i}{t}$, meaning that the error rate is related to the selected time slot.
Thus, to simulate a quantum system with respect to a time slot $t$, one can select a large $n$ to consecutively apply the exponent $\sapp{\cn{exp}({\frac{A}{n}})}{\cn{exp}({\frac{B}{n}})}$ to the state $n$ times, so $\frac{t}{n}$ is very small one such that the error rate $O({(\frac{t}{n})}^2)$ is negligible.
Such tactics can be generalized to arbitrary numbers of summation terms.
For example, to simulate $\hat{H}_{I1}$ with a time slot $t$ through the pick of a splitting number $n$, we compute the exponent $\eexp{\sapp{\hat{H}_{I1}}{t}}$ using the approximation of product formula as the follows.

{\small
\begin{center}
$\eexp{\sapp{\hat{H}_{I1}}{t}}
= \left(\eexp{\sapp{(\sum_{j} \sapp{Z(j)}{Z(j\splus 1)} + z_h \sum_j X(j))}{\frac{t}{n}}}\right)^n
= \left(\sapp{\sapp{\eexp{\sapp{\sapp{Z(1)}{Z(2)}}{\frac{t}{n}}}}{...}}{\sapp{\eexp{\sapp{X(1)}{\frac{t}{n}}}}{...}} \right)^n
$
\end{center}
}

In the Bloch qubit sphere interpretation \cite{mike-and-ike}, the rotation gate $\cn{Rx}$, $\cn{Ry}$, $\cn{Rz}$ can be expressed as some exponents of Pauli matrices, which essentially suggests that the simulation of singleton Pauli $X$, $Y$, and $Z$ terms are the above phase rotation gates, respectively. An $z$-axis interaction exponent $\eexp{\sapp{\sapp{Z(j)}{Z(j\splus 1)}}{\frac{t}{n}}}$ represents a series of quantum gate applications. Their quantum gate representations are summarized as the follows.

{\small
\begin{center}
$
\eexp{\sapp{X(j)}{\frac{t}{n}}}=\cn{Rx}(\frac{2t}{n})(j)
\qquad
\eexp{\sapp{\sapp{Z(j)}{Z(j\splus 1)}}{\frac{t}{n}}}=\cn{CX}(j,j\splus 1);\,\cn{Rz}(\frac{t}{n})(j\splus 1);\,\cn{CX}(j,j\splus 1)
$
\end{center}
}

Here, $\cn{Rx}(\theta)(j)$ and $\cn{Rz}(\theta)(j)$ are $x$-axis and $z$-axis phase rotation gates, rotating $\theta$ angle, applying to $j$-th qubit, and $\cn{CX}(j,j\splus 1)$ controls on $j$-th qubit and applies an $X$ gate to $j\splus 1$-th qubit.
In the end, the simulation of the whole system is a series of applications of the above two gate combinations.
As we mentioned, a quantum computer is essentially a Hamiltonian simulator, where every gate is simulated on a Hamiltonian with respect to some time slots.
The implementations of the above gates are through a series of small gate simulations. Such implementations might not be an effective way of utilizing quantum computers.
In \Cref{sec:compilation}, we can see that a way of directly compile the problem Hamiltonian, such as $\hat{H}_{I1}$, to the machine Hamiltonian that a quantum computer supports,
which might produce a more effective way of compilation.

This section provides an overview of the \qsnd system, starting with the datatypes in the system.
As we mentioned, the definition of a Hamiltonian in second quantization relies on a lattice model showing the relative positions of particles,
each particle of which lives in a lattice site.

We first describe the state structure and operations of a singleton particle. The \qsnd single particle state structures and types are given in \Cref{fig:data}.
Each particle state represents a quantum state snapshot of the number of electrons occupying the practice site,
and it can be expressed as a dual Hilbert space $\hspb{n}$, a.k.a., a pair of $n$ dimensional Hilbert spaces.

In \qsnd, each single particle state $\sum_j\dualm{z_j}{k_j}{m_j}$ is linear combination of basis-kets $\dualm{z_j}{k_j}{m_j}$.
Each basis-ket consists with a complex amplitude value $z$, and two basis vectors $\ket{k}_{\uparrow}$ and $\ket{m}_{1}$ with two natural numbers $s$ and $m$ \footnote{Many literature works describe their systems using basis-ket symbols $\ket{\uparrow}$, $\ket{1}$, and $\ket{0}$, which are respectively represented as $\dualm{}{1}{0}$, $\dualm{}{0}{1}$, and $\dualm{}{0}{0}$ in \qsnd.}. The basis-ket formalism is extended from the one in Dirac notation \cite{Dirac1939ANN}, by marking a ket, e.g., $\ket{k}$. with spinning flags ($\uparrow$ and $1$).
Each state is associated with a single particle type $\hspb{n}$ and the basis-vector numbers $k$ and $m$ is in the range $[0,n)$. For example, a basis vector in a two dimensional dual Hilbert space can be in one of the two vectors: $\ket{0}$ and $\ket{1}$.

The spinning operator ($\sigma$) represents the spinning state of a particle, potentially being in up ($\uparrow$) and down ($1$) positions.
For example, $\dualm{}{1}{0}$ (in some literature, $\ket{\uparrow}$) means that a particle site containing a spun-up electron, while $\dualm{}{0}{1}$ (in some literature, $\ket{1}$) refers to 
a particle site containing a spun-down electron.
Sometimes, users intend to ignore the spinning operators in their analyses. In such cases, we assume the particles are always spun-up ($\dualm{z}{k}{0}$) and abbreviate the state as $z\ket{k}$.
%In some particle analyses, researchers need to discuss the spinning ($\sigma$) of particles, typically in up ($\uparrow$) and down ($1$) positions. Usually, the particle spinning is analyzed separately by a pair of Hilbert spaces, which is captured by our dual space design.
In \qsnd, we include a zero state value $\zero$, admitting identity equational property ($\zero + v = v$); explained shortly below.

A single particle operation in second quantization represents the potential of the modification of electrons in a particle site (state snapshot), analogous to the increments or decrements of basis vector numbers in a basis-ket. Typically, a creation operation ($a^{\dag}$) increments the basis vector number and a annihilator ($a$) decrements the basis vector number.
Each single particle operation is also labeled with spinning flags ($a_{\uparrow}$ and $a_{1}$) to manipulate the spun-up and -down basis vectors of a basis-ket, respectively.
The annihilator application semantics on a single basis-ket is summarized as rules \rulelab{S-AUB}, \rulelab{S-AUN}, \rulelab{S-ADB}, and \rulelab{S-ADN} in \Cref{fig:sem}.
An annihilator, with a specific spinning flag $\sigma$, reduces the basis vector number in the specific ket, with the same flag $\sigma$, if the number is not $0$;
otherwise, the application results in a zero state ($\zero$).
The above rules are applied to single basis-kets (without amplitude values). In general, applying such an operation to a quantum state that might be in superposition (a linear combination of basis-kets), results in a linear combination of applying the operation to different singleton basis-kets.
In contrast, we can view a creator ($\sdag{a}_{\sigma}$) as the increment of basis vectors, as its application on a basis-ket can be summarized as follows.
Each creator application is associated with the $n$ value from the type ($\hspb{n}$) of the state that the creator is applied to.

{\small
\begin{center}
$
\begin{array}{l@{\;\;}c@{\;\;}l@{\qquad}l@{\;\;}c@{\;\;}l}
\sdag{a}_{\uparrow}\dualm{}{k}{m} &\longrightarrow&\zero
&
\sdag{a}_{1}\dualm{}{k}{n} &\longrightarrow&\zero
\\[0.8em]
\sdag{a}_{\uparrow}\dualm{}{k}{m} &\longrightarrow& \dualm{}{k\splus 1}{m}
\;
\cn{if}\;k\neq n
&
\sdag{a}_{1}\dualm{}{k}{m} &\longrightarrow& \dualm{}{k}{m\splus 1}
\;
\cn{if}\;m\neq n
\end{array}
$
\end{center}
}

Note that \qsnd models the second quantization operations by using only annihilators ($a$) and defines a creator as the transpose ($\sdag{e}$) of an annihilator; see \Cref{sec:formal}.

The above \qsnd data and operation definitions are suitable for formalizing the behavior of a single particle site.
To connect different particles, we utilize a tensor operation $\otimes$, i.e., $v_1 \otimes v_2$ connects two single particle data and $e_1 \otimes e_2$ connects two operations.
For example, the composition of two particle, states can be expressed as $v\otimes v'$, and we adapt the follow abbreviation.

{\small
\begin{center}
$
\dualm{}{k_1}{m_1}\otimes\dualm{}{k_2}{m_2} = \dualm{}{k_1}{m_1}\dualm{}{k_2}{m_2}
\qquad
\sum_j z_j\eta_j\otimes\sum_k z_k\eta_k = \sum_{j,k} (z_j * z_k) \eta_j\eta_k
$
\end{center}
}

In the case of expression entangled quantum states across different particles, we denote the $n$ particle state form to be: $\sum_j z_j \eta_{1j}\eta_{2j} ... \eta_{nj}$, an extension of a Dirac notation with spinning flags.
Essentially, a tensor product can be viewed as a location separation in a system. Applying a tensor product of operations to a state is to apply each operation to the right location in every basis-ket in the state. For example, $a_{\uparrow} \otimes \sdag{a}_{1}$ can be understood as applying the first annihilator ($a_{\uparrow}$) to the first particle site and the creator ($\sdag{a}_{1}$) applies to the second particle. If the state is the one above ($\sum_{j,k} (z_j * z_k) \eta_j\eta_k$), the application will be:

{\small
\begin{center}
$
\sapp{(a_{\uparrow} \otimes \sdag{a}_{1})}{(\sum_{j,k} (z_j * z_k) \eta_j\eta_k)} \longrightarrow \sum_{j,k} (z_j * z_k) (\sapp{a_{\uparrow}}{ \eta_j}) (\sapp{\sdag{a}_{1}}{ \eta_k})
$
\end{center}
}


Additionally, we permit a linear sum operation $e_1+e_2$, performing a linear sum, i.e., applying $e_1+e_2$ to a state $v$ means $(\sapp{e_1}{v}) + (\sapp{e_2}{v})$.
A sum operation might produce superposition if $v$ is a state just initialized as a tensor product of basis-kets,
which can be thought as a \emph{quantum choice} operation, in the sense that one can perform either $e_1$ or $e_2$ to the state $v$ at the same time.
We also permit a function sequencing operation $\sapp{e_2}{e_1}$, consecutively applying $e_1$ and $e_2$ to a state. Essentially, the sequencing operator $\sapp{e_2}{e_1}$ is an abbreivation of $\lambda x . \sapp{e_2}{(\sapp{e_1}{x})}$ where $x$ is a state. More information is in \Cref{sec:formal}.

%\liyi{restruct the following, so we can talk about the meaning of X, Y, Z as another way of representation. We need to discuss the meaning of JW transformation in depth.}
\myparagraph{Connects to Quantum Operations.}
Here, we link \qsnd, a quantum mechanics second quantization formalism, with circuit-based quantum computing.
As we mentioned, a Hamiltonian definition represents a snapshot of the potential quantum movement of particles located in different lattice sites.
A major computation is to calculate the energy state according to the formula in \Cref{sec:background}.
Another application is to take the matrix exponential of the Hamiltonian, a.k.a., Hamiltonian quantum simulation,
analogous to automatically generating a movie based on a given snapshot.
Quantum simulation and circuit-based quantum computers are essentially two viewpoints of the same thing,
and circuit-based quantum computers are implemented in quantum simulators \cite{Tacchino_2019,Li_2022}.
To show how a quantum computer is connected to Hamiltonian simulation, we first show how Pauli groups can be defined in terms of \qsnd.
Pauli groups are given as follows:

{\small
\[
I \triangleq  
\begin{bmatrix}
1 & 0\\
0 & 1
\end{bmatrix}
\qquad
X \triangleq  
\begin{bmatrix}
0 & 1\\
1 & 0
\end{bmatrix}
\qquad
Y \triangleq  
\begin{bmatrix}
0 & \sminus i\\
i & 0
\end{bmatrix}
\qquad
Z \triangleq  
\begin{bmatrix}
1 & 0\\
0 & \sminus 1
\end{bmatrix}
\]
}

The meaning of Pauli groups in terms of second quantization is different from gates appearing in a quantum circuit.
They provide a different view of particle movements in a snapshot, i.e., instead of describing electron occupation by creators and annihilators,
Pauli groups describe particle movements as spinning rotation bases of particles across $X$, $Y$, and $Z$ bases \footnote{More specifically, Pauli groups are the bases in Lie algebra for defining the spinning in $X$, $Y$, $Z$ directions \cite{Samelson1969NotesOL}.}.
We show below the transformation from creators and annihilators to Pauli group bases, for a single particle, through the Jordan-Wigner transformation \cite{JordanAboutTP} as follows.
The transformation is a simplified version, with \emph{only} showing the spun-up portion and  \emph{omitting} the spun-down parts.
The matrix representations of creators ($a$) and annihilators ($\sdag{a}$) are given as $\begin{psmallmatrix}
0 & 0\\
1 & 0
\end{psmallmatrix}$ and $\begin{psmallmatrix}
0 & 1\\
0 & 0
\end{psmallmatrix}$, respectively.

{\small
\[
I = \sapp{\sdag{a}}{a} + \sapp{a}{\sdag{a}} 
\qquad
\qquad
X = \sdag{a} + a
\qquad
\qquad
Y = i a - i \sdag{a}
\qquad
\qquad
Z = \sapp{\sdag{a}}{a} - \sapp{a}{\sdag{a}} 
\]
}

Here, $i$ is a complex amplitude value, and $i a - i \sdag{a}$ is an abbreviation of $\sapp{\sdag{a}}{a} + (\sapp{\sminus a}{\sdag{a}})$.
To understand the transformation, recall that a Hamiltonian represents a snapshot showing the potential movement of a particle.
Defining the $X$, $Y$, and $Z$ bases in a second quantization formalism is to identify three different orthonormal bases so that one can define operations through a linear combination of the three different bases that represent three different ways of potential movements.
The transformation first defines the $X$ basis to be a sum of a creator and annihilator.
If we view a sum operation as a quantum choice, the $X$ basis transformation refers to that a potential movement in an $X$ basis is to either create or annihilate an electron.
To define the $Y$ basis, the transformation tries to a orthonormal basis with respect to $X$;
one trivial case is to define $Y$ as the complex counterpart of $X$, which results in the $Y$ transformation above.
The transformation of $Z$ basis is to identify a third orthonormal basis other than $X$ and $Y$.
Here, we play some trick based on the matrix formation of creators and annihilators.
In the matrix form, $\sapp{\sdag{a}}{a}$ produces $\begin{psmallmatrix}
0 & 0\\
0 & 1
\end{psmallmatrix}$ and $\sapp{a}{\sdag{a}}$ produces $\begin{psmallmatrix}
1 & 0\\
0 & 0
\end{psmallmatrix}$, which is orthonormal with respect to the creators and annihilators; thus, the Jordan-Wigner transformation $Z$ to be a linear combination of the two matrices.
An example usage of the Pauli group system is the $Z$-basis interactions in the Ising model in \Cref{sec:formal}.

In a quantum computer, circuit gates are essentially implemented as the simulation of a gate Hamiltonian with respect to a certain time slot,
i.e., to define a gate $U$, one first performs a reversed engineering, computes the eigendecomposition of $U$'s unitary matrix,
forms $U$'s Hamiltonian $\hat{H}_U$ based on the eigenstates found in the eigendecomposition \footnote{It is not necessary to perform Hamiltonian simulation by constructing the Hamiltonian through eigenstates, but the simulation of a quantum gate in a computer might require the Hamiltonian is fixed during the simulation, so it is better to form the Hamiltonian based on eigenstates.},
and simulates the gate based on the Schrodinger equation, $\eexp{\hat{H}_U t}$.
Here, we show the simulation of a Hadamard (\cn{H}) and controlled-not (\cn{CX}) gate, as we assume that the simulation time slot is $\pi$.

{
\begin{center}
$
\hat{H}_{\cn{H}} = (\frac{1}{2}\sminus\frac{\sqrt{2}}{4}) \sapp{a}{\sdag{a}} + (\frac{1}{2}\sminus\frac{\sqrt{2}}{4}) \sapp{\sdag{a}}{a}+{(\sminus\frac{\sqrt{2}}{4})}X
\qquad
\qquad
\cn{H}=\eexp{ \hat{H}_{\cn{H}} \pi}
$
\end{center}
}

The above formula is the Hamiltonian for simulating a Hadamard gate ($\cn{H}$).
To reversely engineers the Hamiltonian, we perform an eigendecomposition on the Hadamard gate, find out one of the eigenstates is $\varphi = -\sin(\frac{\pi}{8})\ket{0}+\cos(\frac{\pi}{8})\ket{1}$,
and constructs the above Hamiltonian based on the eigenstate.
The above Hamiltonian is the second quantization form of the matrix $\sapp{\varphi}{\sdag{\varphi}}$ \footnote{$\sapp{\varphi}{\sdag{\varphi}}=\begin{psmallmatrix}
\frac{1}{2}\sminus\frac{\sqrt{2}}{4} & \sminus\frac{\sqrt{2}}{4}\\
\sminus\frac{\sqrt{2}}{4} & \frac{1}{2}\splus\frac{\sqrt{2}}{4}
\end{psmallmatrix}$}.
A Hadamard gate (\cn{H}) can be defined as a simulation of the above Hamiltonian as $\cn{H}=\eexp{ \hat{H}_{\cn{H}} \pi}$, with the time slot $\pi$.

{
\begin{center}
$
\hat{H}_{\cn{CX}} = \sapp{a}{\sdag{a}} \otimes ((\sminus \frac{1}{2}) X + \frac{1}{2} I)
\qquad
\qquad
\cn{CX}=\eexpa{-i \hat{H}_{\cn{CX}} \pi}
$
\end{center}
}

Similarly, we can also find the Hamiltonian by computing the eigendecomposition of a controlled-not gate (\cn{CX}) and implement it in \qsnd as the formula above.
Then, the gate can be defined as a simulation of the above Hamiltonian as $\cn{CX}=\eexpa{-i \hat{H}_{\cn{CX}} \pi}$, where we define the time slot to be $\pi$.

As the matrix exponential operation turns a Hamiltonian snapshot to a quantum system simulation,
a matrix logarithm operation, modeled in \qsnd, reverses a simulation to a Hamiltonian snapshot.
For example, by applying a matrix logarithm on the $\cn{H}$ and $\cn{CX}$ gates, $\hat{H}_{\cn{H}}$ and $\hat{H}_{\cn{CX}}$ could be one of the results \footnote{Matrix logarithm is not unique. \qsnd fixes the uniqueness by picking one way of implementing the operation. However, the \qsnd type system and equivalence relations are general enough without relying on the specific implementation.}.

\end{comment}

%The Hubbard model is a prime candidate for simulation on quantum computers due to its complexity and difficulty solving it using classical methods. Quantum algorithms, such as the Variational Quantum Eigensolver (VQE), can be employed to find the ground state energy of the system, offering insights into strongly correlated electronic systems. This example demonstrates how the Hubbard model can be used to study the properties of materials and develop new quantum technologies.

\begin{comment}

In the Hubbard model, electrons within the lattice structure experience competing forces: one pushes them to tunnel through an energy barrier to hop to another lattice site (kinetic energy), and the other accounts for on-site interactions such as electron correlations. These two interactions allow the Hamiltonian (energy expression) to be written as the sum of two terms: one for the kinetic energy due to tunneling, and the other for the on-site interactions.

In the Hamiltonian, the indices of the sites describe a 1D lattice system, where \(j\) is adjacent to \(j-1\) and \(j+1\). An index in an operator, such as \(j\) in \(\hat{c}_{j\sigma}^\dagger\), is syntactic sugar for the tensor composition (\(\otimes\)) of identities \(I\). For example, if there are three particles in the system and \(j=2\), the term \(\hat{c}_{j\sigma}^\dagger\) expresses \(I \otimes \hat{c}_{\sigma}^\dagger \otimes I\).

A sequencing operator, e.g., \(\hat{c}_{j\sigma}^\dagger \hat{c}_{j+1\sigma}\), represents an interaction between the two particles at adjacent sites \(j\) and \(j+1\). The expression \(\hat{c}_{j\sigma}^\dagger \hat{c}_{j+1\sigma}\) means that the annihilation of an electron at site \(j+1\) is associated with the creation of an electron with the same spin (\(\sigma\)) at site \(j\). A sequencing operator with two terms applying to the same site, e.g., \(U \hat{c}_{j\uparrow}^\dagger \hat{c}_{j\uparrow} \hat{c}_{j\downarrow}^\dagger \hat{c}_{j\downarrow}\), represents the on-site interaction energy.

In this context, a sequence operation can be viewed as syntactic sugar for a lambda term, \(\lambda x. e_2(e_1(x))\). Summations are syntactic sugars for linear sum operators (\(+\)), allowing for concise representation of interactions. For instance, in the Hubbard model, the term \(\sum_{i, \sigma} \left( \hat{c}_{i\sigma}^\dagger \hat{c}_{i+1\sigma} + \hat{c}_{i+1\sigma}^\dagger \hat{c}_{i\sigma} \right)\) can be expanded as:

\[
(\lambda x. (I \otimes \hat{c}_{\uparrow}) ((\hat{c}_{\uparrow}^\dagger \otimes I) x)) + (\lambda x. (\hat{c}_{\uparrow} \otimes I) ((I \otimes \hat{c}_{\uparrow}^\dagger) x)) + (\lambda x. (I \otimes \hat{c}_{\downarrow}) ((\hat{c}_{\downarrow}^\dagger \otimes I) x)) + (\lambda x. (\hat{c}_{\downarrow} \otimes I) ((I \otimes \hat{c}_{\downarrow}^\dagger) x))
\]

The Hubbard model is a prime candidate for simulation on quantum computers due to its complexity and the difficulty of solving it using classical methods. Quantum algorithms, such as the Variational Quantum Eigensolver (VQE), can be employed to find the ground state energy of the system, offering insights into strongly correlated electronic systems. This example demonstrates how the Hubbard model can be used to study the properties of materials and develop new quantum technologies.

\subsection*{Example: 1D Chain of Hydrogen Atoms}

To illustrate the Hubbard model, consider the example of a one-dimensional ($1D$) chain of hydrogen atoms. The hydrogen atom is chosen for simplicity because it has only one electron per atom, allowing us to focus on the basic interactions without the complexity of multiple electrons per site. The Hamiltonian for the $1D$ hydrogen atom chain can be expressed as:

\[
\hat{H} = -t \sum_{j,\sigma} \left( \hat{c}_{j\sigma}^\dagger \hat{c}_{j+1\sigma} + \hat{c}_{j+1\sigma}^\dagger \hat{c}_{j\sigma} \right) + U \sum_j \hat{n}_{j\uparrow} \hat{n}_{j\downarrow}
\]

where \(t\) represents the hopping integral and \(U\) represents the electron repulsion. The indices \(j\) and \(j+1\) denote adjacent sites in a $1D$ lattice, with \(j\) representing a specific site and \(j+1\) its neighboring site.
\liyi{Below is suject to change. Chandeepa, we will describe the H-chain here instead of Hubbard model, and show a simulation.}
As discussed above, quantum computers perform simulations by executing quantum gates. One of the key tasks of quantum computers is to simulate particle systems. Compiling these systems into circuit gates might produce tens of thousands of gates, each simulated as described earlier.

One significant advantage of using a quantum language based on second quantization is that it allows for direct compilation of Hamiltonians, which are defined for simulating physical systems, into Hamiltonians designed for execution on a quantum computer. This direct compilation translates the simulation of a complex problem Hamiltonian into simulations of simpler Hamiltonians, bypassing the circuit-level transformation. This can potentially lead to more effective optimizations and better error management due to a cleaner compilation goal.

Here, we illustrate this with the Hubbard model.

The Hubbard model is an approximate model used to describe the interactions between electrons in a solid, helping to explain properties such as electrical conductivity and magnetism. It has been used to model Heavy Fermion Systems (HFS), where electrons experience competing forces due to strong correlations, and High-Temperature Superconductors (HTS), where the constituent metallic compounds have strong correlations in certain orbitals\footnote{In \(CuO_{2}\), the 3d orbital electrons are strongly correlated.}.

The Hubbard model is most easily and precisely described in 1D systems, or a "chain of atoms" along a single dimension\footnote{Higher dimensional systems may introduce additional interactions not considered in the Hubbard model.}. A single atom may harbor many electrons, leading to multiple on-site interactions. The simplest case to consider is the hydrogen atom, which has only one $s$-orbital permitting up to two electrons, one spin-up and the other spin-down. We restrict our example to describe the one-dimensional hydrogen atom chain, the only configuration analytically solved so far. In this setting, the kinetic energy results from an electron annihilating at one lattice site and creating at another, and the on-site interactions arise from the interaction between two $s$-orbital electrons.

In the Hubbard model, electrons within the lattice structure experience competing forces: one pushes them to tunnel through an energy barrier to hop to another lattice site (kinetic energy), and the other accounts for on-site interactions such as electron correlations. These two interactions allow the Hamiltonian (energy expression) to be written as the sum of two terms: one for the kinetic energy due to tunneling, and the other for the on-site interactions.

In our notation, we use $\sdag{a}_{\sigma}(j)$ to denote the creation operator and $a_{\sigma}(j)$ to denote the annihilation operator, consistent with the expressions used in \qsnd. For instance, in fermionic systems, these operators are represented as $\sdag{\hat{c}}_{j\sigma}$ and $\hat{c}_{j\sigma}$ respectively.

The Hamiltonian for the 1D hydrogen atom chain can be expressed as:
\[
\hat{H} = -z_t \sum_{j,\sigma \in \{\uparrow,\downarrow\}} \left(\sdag{a}_{\sigma}(j) a_{\sigma}(j+1) + \sdag{a}_{\sigma}(j+1) a_{\sigma}(j)\right) + z_u \sum_{j} \sdag{a}_{\uparrow}(j) a_{\uparrow}(j) \sdag{a}_{\downarrow}(j) a_{\downarrow}(j)
\]
where \(z_t\) represents the hopping integral and \(z_u\) represents the electron repulsion.

In the above function, the indices of the sites describe a 1D lattice system, where \(j\) is adjacent to \(j-1\) and \(j+1\). In \qsnd, an index in an operator, such as \(j\) in $\sdag{a}_{\sigma}(j)$, is syntactic sugar for the tensor composition ($\otimes$) of identities \(I\). For example, if there are three particles in the system and \(j=2\), the term $\sdag{a}_{\sigma}(j)$ expresses \(I \otimes \sdag{a}_{\sigma} \otimes I\).

A sequencing operator, e.g., $\sdag{a}_{\sigma}(j) a_{\sigma}(j+1)$, represents an interaction between the two particles at adjacent sites \(j\) and \(j+1\). The expression $\sdag{a}_{\sigma}(j) a_{\sigma}(j+1)$ means that the annihilation of an electron at site \(j+1\) is associated with the creation of an electron with the same spin (\(\sigma\)) at site \(j\). A sequencing operator with two terms applying to the same site, e.g., $z_u \sdag{a}_{\uparrow}(j) a_{\uparrow}(j) \sdag{a}_{\downarrow}(j) a_{\downarrow}(j)$, represents the on-site interaction energy.

In \qsnd, a sequence operation $\sapp{e_2}{e_1}$ is syntactic sugar for a lambda term, $\lambda x. \sapp{e_2}{(\sapp{e_1}{x})}$. Summations are syntactic sugars for linear sum operators ($+$), allowing for concise representation of interactions. For instance, in the Hubbard model, the term $\sum_{i,\sigma \in \{\uparrow,\downarrow\}} \left(\sdag{a}_{\sigma}(i) a_{\sigma}(i+1) + \sdag{a}_{\sigma}(i+1) a_{\sigma}(i)\right)$ can be expanded as:
\[
(\lambda x. (I \otimes a_{\uparrow}) ((\sdag{a}_{\uparrow} \otimes I) x)) + (\lambda x. (a_{\uparrow} \otimes I) ((I \otimes \sdag{a}_{\uparrow}) x))
+ (\lambda x. (I \otimes a_{\downarrow}) ((\sdag{a}_{\downarrow} \otimes I) x)) + (\lambda x. (a_{\downarrow} \otimes I) ((I \otimes \sdag{a}_{\downarrow}) x))
\]

This example demonstrates how the Hubbard model can be used for quantum system simulation. It highlights the advantages of using second quantization and \qsnd for efficiently describing and simulating complex quantum systems.

\end{comment}

\begin{comment}
\myparagraph{Quantum System Simulation and Hubbard Model.}\label{sec:hubbard}
As we can see above, quantum computers essentially perform simulations on individual gates.
One of the key tasks of quantum computers is to simulate particle systems.
Compiling the systems into circuit-gates might produce tens of thousands of gates, each of which is simulated through the above procedure.
One key advantage of using a new quantum language based on second quantization is that we can directly compiling the Hamiltonian, defined for simulating a system, to Hamiltonians, designed in a quantum computer for execution. This direct compilation essentially means that we translate the simulation of a problem Hamiltonian to the simulations of some simpler Hamiltonians,
which helps us bypass the circuit-level transformation, with the potentials of effective optimizations and better error management due to a cleaner compilation goal.
Here, we show a simple example through the Hubbard model.

The Hubbard model is one of the approximate models to describe the interactions between electrons in a solid, thus facilitating the explanation of properties such as electrical conductivity and magnetism. In fact, it has been used to model Heavy Fermion Systems (HFS) where electrons experience competing forces due to a strong correlation between them against tunneling and, to model High-Temperature Superconductors (HTS) where the constituent metallic compound has strong correlations in one of the orbitals\footnote{In $CuO_{2}$ the 3d orbital electrons are strongly correlated.}.\par

\liyi{
The Hubbard model is most easily and precisely described in 1D systems, or a ``chain of atoms'' along a single dimension as it is usually called\footnote{Higher dimensional systems may introduce additional interactions due to effects that are not considered under the Hubbard model.}. A single atom may harbor many electrons and therefore will have multiple on-site interactions between them. The simplest atom that can be considered is the hydrogen atom, where there is only one 
$s$-orbital, which permits up to 2 electrons, one spin-up and the other spin-down. Thus, we restrict our example to describe the only configuration to be analytically solved so far, i.e., the one-dimensional hydrogen atom chain. In this setting, the kinetic energy is due to an electron annihilating at a certain lattice site and creating at another, and the on-site interactions originate only due to the interaction between two $s$-orbital electrons. Additionally, we alter the conventional notation of the terms to resemble the exact notation we use in \qsnd expressions as follows.
}

A postulate in the Hubbard model that should be vaguely evident from the example use cases mentioned above is that the electrons within the lattice structure experience competing forces, one of which pushes them to tunnel through an energy barrier to hop to another lattice site and another which accounts for on-site interactions such as the correlations described. These two interactions allow the Hamiltonian (i.e., the energy expression) to be written as the addition of two terms, in which one of them (conventionally, the first) represents the kinetic energy due to tunneling whereas the other (typically the second) represents the on-site interactions.\par

The Hubbard model is most easily and precisely described in 1D systems, or a ``chain of atoms'' along a single dimension as it is usually called\footnote{Higher dimensional systems may introduce additional interactions due to effects that are not considered under the Hubbard model.}. A single atom may harbor many electrons and therefore will have multiple on-site interactions between them. The simplest atom that can be considered is the hydrogen atom, where there is only one 
$s$-orbital, which permits up to 2 electrons, one spin-up and the other spin-down. Thus, we restrict our example to describe the only configuration to be analytically solved so far, i.e., the one-dimensional hydrogen atom chain. In this setting, the kinetic energy is due to an electron annihilating at a certain lattice site and creating at another, and the on-site interactions originate only due to the interaction between two $s$-orbital electrons. Additionally, we alter the conventional notation of the terms to resemble the exact notation we use in \qsnd expressions as follows.
\begin{itemize}
    \item In fermionic systems, the creation and annihilation operators are represented by $\sdag{\hat{c}}_{j\sigma}$. In our notation, we use $\sdag{a}_{\sigma}(j)$ to identically denote the same operators without an alteration in the definition and its semantics. The latter resembles expressions used in \qsnd.
\end{itemize}\par

\chand{Can we use $k_{t}$ and $k_{u}$ for the hopping integral term and the on-site interaction strength term respectively? In the usual notation of the fermionic systems (which we are discussing in this work), the letter $c$ (with appropriate subscripts) denotes creation/annihilation operators. This might not be confusing for our intended audience, but in case someone with a physics background reads it, they might glance over these parts and assume the usual notation.}

\chand{Can we use $\sdag{a}(j,\sigma)$ instead of $\sdag{a}_{\sigma}(j)$? It seems more compliant with the functional notation.}

Subsequently, the Hamiltonian for 1D hydrogen atom chain can be given as,
{
\begin{center}
$
\hat{H} = \sminus z_t \sum_{j,\sigma\in\{\uparrow,\downarrow\}}(\sdag{a}_{\sigma}(j) a_{\sigma}(j\splus 1) + \sdag{a}_{\sigma}(j\splus 1) a_{\sigma}(j))+z_u \sum_{j} \sdag{a}_{\uparrow}(j) a_{\uparrow}(j)\sdag{a}_{\downarrow}(j) a_{\downarrow}(j)
$
\end{center}
}

\chand{TODO (for Chandeepa): Modify the following content to follow the introduction content above. Liyi, check the Review tab of overleaf for my suggestions and comments.}

\liyi{Show 2D in Ising model. point to people that 2D is definable in our system in Ising model. Hubrbard model here, and Ising model in section 4. }

\liyi{link to some Hurbard model simulation gates circuit diagram, link to the citation. why not just simiulate the model directly.}

\chand{Possible change in this sentence} Here, $z_t$ and $z_u$ are some constant numbers \footnote{$z_t$ represents hopping integral and $z_u$ represents electron repulsion.}. 
As we mentioned, second quantization formulas are usually associated with the lattice concept, where particle sites are managed as points in a coordinate system.
The above function describes an $1D$ lattice (coordinate) system, in the sense that the indices of the site describes a line structure, where $j$ is adjacent to $j\sminus 1$ and $j\splus 1$.
In \qsnd, an index in an operator, e.g., the $j$-th index in $\sdag{a}_{\sigma}(j)$, is a syntactic sugar of the tensor composition ($\otimes$) of identities $I$.
For example, if there are three particles in the system and $j=2$, the term $\sdag{a}_{\sigma}(j)$ expresses $I\otimes \sdag{a}_{\sigma}\otimes I$. 
Despite the absence of analytical solutions, note that \qsnd is suitable for describing arbitrary lattice systems, due to our underlining $\lambda$-calculus system, e.g., one can encode a $3D$ lattice system by implementing it as a three dimensional array structure in $\lambda$-calculus, with the array separator using the tensor operator ($\otimes$).

A sequencing operator, e.g., $\sdag{a}_{\sigma}(j) a_{\sigma}(j\splus 1)$, is essentially a matrix multiplication. A sequencing operator applying to two adjacent particle sites, e.g., $j$ and $j\splus 1$, represents an interaction between the two particles. The expression $\sdag{a}_{\sigma}(j) a_{\sigma}(j\splus 1)$ means that the annihilation of an electron in the $j \splus 1$ site is associated with the creation of an electron, with the same spin ($\sigma$), in the $j$-th site.
A sequencing operator with two children (AST...) applying to the same site, e.g., $\sapp{\sdag{a}_{\downarrow}(j)}{ a_{\downarrow}(j)}$, usually refers to adding a pre-computed constant, e.g., $z_u$, to a certain state. For example, $z_u \sdag{a}_{\uparrow}(j) a_{\uparrow}(j)\sdag{a}_{\downarrow}(j) a_{\downarrow}(j)$ adds the constant $z_u$ to the $j$-th site if the basis-ket state is $\dualm{}{1}{0}$ or $\dualm{}{0}{1}$.

Usually, a quantum physical model is symmetric, e.g., users probably want to talk about interactions between every two adjacent particles. most of the models .... \liyi{Chandeepa, fixed here. }
The linear sum operator ($+$) represents a choice operator allowing users to define such symmetry. In the above formula, the term $\sdag{a}_{\sigma}(j) a_{\sigma}(j+1) + \sdag{a}_{\sigma}(j+1) a_{\sigma}(j)$
describes that the interaction can be either an action in the $(j\splus 1)$-th site followed by one in the $j$-th site, or an action in the $j$-th site following by one in the $(j\splus 1)$-th site. \liyi{Chandeepa, please fixed it. }

\chand{We have not described the second term for electron-electron repulsions. It adds up the total number of orbitals in which it is doubly occupied (two electrons occupying the same orbitals but with opposite spins) and multiplies by the energy per each doubly occupied orbital ($U$) to collectively represent the total energy due to electron-electron interactions.}

As we mentioned above, a sequence operation $\sapp{e_2}{e_1}$ is a syntactic sugar of a lambda term, $\lambda x . \sapp{e_2}{(\sapp{e_1}{x})}$.
Additionally, summations are syntactic sugars for linear sum operators ($+$) in \qsnd, e.g., if there are two particles in the Hubbard model, the term $\sum_{i,\sigma\in\{\uparrow,\downarrow\}}(\sdag{a}_{\sigma}(i) a_{\sigma}(i+1) + \sdag{a}_{\sigma}(i+1) a_{\sigma}(i))$ expresses the following.

{\small
\begin{center}
$
 (\lambda x. (I\otimes a_{\uparrow}) ((\sdag{a}_{\uparrow}\otimes I) x)) + (\lambda x. (a_{\uparrow}\otimes I) ((I\otimes \sdag{a}_{\uparrow}) x))
 +
  (\lambda x. (I\otimes a_{\downarrow}) ((\sdag{a}_{\downarrow}\otimes I) x)) + (\lambda x. (a_{\downarrow}\otimes I) ((I\otimes \sdag{a}_{\downarrow}) x))
$
\end{center}
}

\liyi{Showing an example of simulation by using Habbard model.}

\end{comment}











